Symmetric Monoidal Smash Products in Homotopy Type Theory

In Homotopy Type Theory, few constructions have proved as troublesome as the smash product. While its definition is just as direct as in classical mathematics, one quickly realises that in order to define and reason about functions over iterations of it, one has to verify an exponentially growing number of coherences. This has led to crucial results concerning smash products remaining open. One particularly important such result is the fact that smash products form a (1-coherent) symmetric monoidal product on the universe of pointed types. This fact was used, without a complete proof, by e.g. Brunerie in his PhD thesis to construct the cup product on integral cohomology and is, more generally, a fundamental result in traditional algebraic topology. In this paper, we salvage the situation by introducing a simple informal heuristic for reasoning about functions defined over iterated smash products. We then use the heuristic to verify e.g. the hexagon and pentagon identities, thereby obtaining a proof of symmetric monoidality. We also provide a formal statement of the heuristic in terms of an induction principle concerning the construction of homotopies of functions defined over iterated smash products. The key results presented here have been formalised in the proof assistant Cubical Agda.

==> sections/EMSpaces.tex <==
\section{Eilenberg-MacLane spaces}
\label{sec:EM}

In order to define representable cohomology in HoTT, we will need to
define Eilenberg-MacLane spaces. These are spaces $K(G,n)$ associated
to an abelian\footnote{Technically, this is only needed when $n>1$,
  but in this paper we will for simplicity always assume $G$ to be
  abelian.} group $G$ and a natural number $n$ such that
$\pi_n(K(G,n)) \simeq G$ and all other homotopy groups vanish. These
spaces carry the structure of an h-space which we will later see
induces the group structure on cohomology. We will also see that they
come equipped with a graded multiplication which, also in
Section~\ref{sec:cohomology}, will be lifted to define cohomology
rings.

The definition of Eilenberg-MacLane spaces and their h-space structure
in HoTT is due to \citet{LicataFinster14}. The special case of
integral Eilenberg-MacLane spaces, i.e.\ $K(\bZ,n)$, was considered by
\citet{Brunerie16}, who gave an alternative and very compact
definition in terms of truncated spheres. This definition of
$K(\bZ,n)$ was also considered by \citet{BLM}. In this section we will
generalise the optimised proofs regarding integral Eilenberg-MacLane
spaces and their h-space structure found in~\citep{BLM} to a definition
of general Eilenberg-MacLane spaces following~\citet{LicataFinster14}.

In order to ease the notation when describing the induction principle, we will define $K(G,n)$ one
step at a time. The crucial step is $K(G,1)$, which will be defined in
terms of the following construction.

% \anders{Har K(G,1) definierats i tre steg så här tidigare? Har någon
%   annan använt sig av L?
% --- Nej, men det gör det lättare att beskriva induktionsprincipen}

\begin{definition}
  Given a type $A$, we define $L(A)$ by the HIT
  \begin{itemize}
    \item $\star : L(A)$
    \item $\Loop_k : A \to \star = \star$
    \end{itemize}
\end{definition}

Given a group $G$, the type $L(G)$ is \emph{almost} the first Eilenberg-MacLane
space of $G$. By adding a constructor connecting the group structure
on $G$ with the h-space structure
on $\Omega(L(G))$, we approximate it further.
\begin{definition}[Raw Eilenberg-MacLane spaces]
  We define the first raw Eilenberg-MacLane space, denoted
  $\widetilde{K}(G,1)$, by the following HIT
  \begin{itemize}
  \item $\iota : L(A) \to \widetilde{K}(G,1)$
  \item For every $g_1,g_2 : G$, a filler $\mathsf{sq}(g_1,g_2)$ of the square
    \[\begin{tikzcd}[ampersand replacement=\&]
	\iota(\star) \&\&\& \iota(\star) \\
	\iota(\star) \&\&\& \iota(\star)
	\arrow["{\ap{\iota}{\LoopG{(g_1 + g_2)}}}", from=1-1, to=1-4]
	\arrow["{\ap{\iota}{\LoopG{g_1}}}"', from=2-1, to=2-4]
	\arrow["{\ap{\iota}{\LoopG{g_2}}}"', from=2-4, to=1-4]
	\arrow["{\mathsf{refl}}", from=2-1, to=1-1]
\end{tikzcd}\]
  \end{itemize}
  For $n > 1$, we define $\widetilde{K}(G,n) := {\Sigma
    (\widetilde{K}(G,n-1))}$.
\end{definition}

In practice, we will omit the $\iota$ and simply write e.g.\
$\star : \widetilde{K}(G,1)$ and
$\LoopG{g} : \Omega(\widetilde{K}(G,1))$. We let $0_k$ denote the
basepoint of $\widetilde{K}(G,n)$, i.e.\ $0_k := \star$ when $n=1$ and
$0_k := \north$ when $n>1$.

\begin{definition}[Eilenberg-MacLane spaces]
  Given an integer $n \geq 1$ and an abelian group $G$, we define the
  $n$th Eilenberg-MacLane space by
  $K(G,n) := \truncT{\widetilde{K}(G,n)}_n$. The zeroth
  Eilenberg-MacLane space is simply $K(G,0) := G$.
\end{definition}

The type $K(G,n)$ is pointed by $0_G$ when $n = 0$ and $\trunc{0_k}$
when $n\geq 1$. With some abuse of notation, we will also use $0_k$ to
denote the basepoint of $K(G,n)$.

Eilenberg-MacLane spaces come with important elimination
principles. Let $n \geq 1$, the fundamental elimination principle of
$K(G,n)$ is given in Figure~\ref{elim:KG} and says that, given a
fibration $P : K(G,n) \to \ntype{n}$, any section
$f : (x : K(G,n)) \to P(x)$ is uniquely determined by its action on
canonical elements $\trunc{x} : K(G,n)$, where $x:\widetilde{K}(G,n)$.
%
If $P$ is set-valued and $n = 1$, it suffices to define the section
for elements in $L(G)$---see Figure~\ref{elim:KG-set}. In other words,
we do not need to prove that our construction respects the
$\mathsf{sq}$-constructor.
%
Finally, it is easy to see that if $P$ is a family of $(n-2)$-types,
then any section $(x : K(G,n)) \to P(x)$ is uniquely determined by its
action on the basepoint $0_k : K(G,n)$---see Figure~\ref{elim:KG-triv}.
\todo{Anders är lite förvirrad av vad vi försöker säga här... Lås oss diskutera det --- ändrade lite i diagrammen. Kanske tydligare? -- Inte direkt...}

\begin{figure}[h!]%
    \centering
    \subfloat[\centering $n$-type elimination \label{elim:KG}]{\begin{tikzcd}[ampersand replacement=\&]
	\Sigma_{x : K(G,n)}{P(x)} \\
	{K}(G,n) \& \widetilde{K}(G,n)
	\arrow[from=1-1, to=2-1]
	\arrow["{|-|}", from=2-2, to=2-1]
	\arrow[from=2-2, to=1-1]
	\arrow["{\exists!}", bend left=40, dashed, from=2-1, to=1-1]
  \end{tikzcd}}%
    \qquad
    \subfloat[\centering $0$-type elimination for $K(G,1)$ \label{elim:KG-set}]{\begin{tikzcd}[ampersand replacement=\&]
	\Sigma_{x : K(G,1)}{P(x)} \\
	{K}(G,1) \& L(G)
	\arrow[from=1-1, to=2-1]
	\arrow["{|-|\circ \iota}", from=2-2, to=2-1]
	\arrow[from=2-2, to=1-1]
	\arrow["{\exists!}", bend left=40, dashed, from=2-1, to=1-1]
\end{tikzcd}}%
    \qquad
    \subfloat[\centering $(n-2)$-type elimination \label{elim:KG-triv}]{
      \begin{tikzcd}[ampersand replacement=\&]
	\Sigma_{x : K(G,n)}{P(x)} \\
	{K}(G,n) \& \mathbbm{1}
	\arrow[from=1-1, to=2-1]
	\arrow[from=2-2, to=2-1]
	\arrow[from=2-2, to=1-1]
	\arrow["{\exists!}", bend left=40, dashed, from=2-1, to=1-1]
      \end{tikzcd}}%
    \caption{Elimination principles for $K(G,n)$}%
    \label{fig:example}%
\end{figure}

We will in Section~\ref{sec:omegakgn} see that
$\Omega^n K(G,n) \simeq G$, but before this will establish that it is
$(n-1)$-connected. These two facts imply that $\pi_n(K(G,n)) \simeq G$
and that all other homotopy groups vanish, which therefore shows that
$K(G,n)$ is indeed an Eilenberg-MacLane space.

\begin{proposition}
  \label{prop:K-connected}
  The type $K(G,n)$ is $(n-1)$-connected.
\end{proposition}
\begin{proof}
  We want to show that $\truncT{K(G,n)}_{n-1}$ is contractible.  When
  $n = 0$, the statement is trivial, since $\truncT{A}_{-1}$ is
  contractible for any pointed type $A$. Let $n \geq 1$, we choose the
  centre of contraction to be $\KO$. We now want to construct
  a section $(x : \truncT{K(G,n)}_{n-1}) \to \KO = x$. Since
  $\truncT{K(G,n)}_{n-1}$ is an $(n-1)$-type, all path types over it
  are $(n-2)$-types. Thus, it suffices to construct the section over
  $\KO$, which is trivial by $\refl : \KO =
  \KO$.
\end{proof}

The type ${K}(G,n)$ is functorial in $G$, i.e.\ for any homomorphism
$\phi : G_1 \to G_2$, we have an induced map $\phi_n : K(G_1,n) \to
K(G_2,n)$. We define this as a map
$\widetilde{K}(G_1,n) \to \widetilde{K}(G_2,n)$. When $n = 0$, we set
$\phi_0 := \phi$. For $n = 1$, $\phi_1$ is defined by
\begin{align*}
  \phi_1(\star) &:= \star \\
  \ap{\phi_1}{\LoopG{g}} &:= \LoopG{\phi_0(g)}
\end{align*}


This respects the $\mathsf{sq}$ constructor of $\widetilde{K}(G_1,n)$
since $\phi$ is assumed to be a homomorphism. For $n \geq 2$, we
define it recursively using functoriality of $\Sigma$ and the fact
that $\widetilde{K}(G,n) := {\Sigma (\widetilde{K}(G,n-1))}$:

\begin{center}
\begin{tikzcd}[ampersand replacement=\&]
	{\widetilde{K}(G_1,n)} \&\& {\widetilde{K}(G_2,n)} \\
	{\Sigma(\widetilde{K}(G_1,n-1))} \&\& {\Sigma(\widetilde{K}(G_2,n-1))}
	\arrow[Rightarrow, no head, from=1-1, to=2-1]
	\arrow["{\Sigma(\phi_{n-1})}", from=2-1, to=2-3]
	\arrow["{\phi_n}", dashed, from=1-1, to=1-3]
	\arrow[Rightarrow, no head, from=1-3, to=2-3]
\end{tikzcd}
\end{center}

We also remark that there is a map
$\sigma_n : K(G,n) \to \Omega(K(G,n+1))$. We define it for raw
Eilenberg-MacLane spaces by
%
\begin{align*}
  \sigma_n(x) :=\begin{cases} \LoopG{g} & \text{ if $n = 0$}\\
  \merid{x} \cdot (\merid{0_k})^{-1} &\text{ otherwise}
  \end{cases}
\end{align*}
%
As $\Omega(K(G,n+1))$ is an $n$-type, this definition also induces, via $n$-type elimination for Eilenberg-MacLane spaces (see Figure~\ref{elim:KG}),
a map $K(G,n) \to \Omega(K(G,n+1))$:
\begin{center}
\begin{tikzcd}[ampersand replacement=\&]
	{\widetilde{K}(G,n)} \&\& {\Omega(\widetilde{K}(G,n+1))} \& {\Omega(K(G,n+1))} \\
	{K(G,n)}
	\arrow["{\sigma_n}", from=1-1, to=1-3]
	\arrow["{\mathsf{ap}_{\trunc{-}}}", from=1-3, to=1-4]
	\arrow[from=1-1, to=2-1]
	\arrow[dashed, from=2-1, to=1-4]
\end{tikzcd}
\end{center}
With some abuse of
notation, we also denote this map by $\sigma_n$. The following fact follows immediately by construction of $\sigma_n$.
\begin{lemma}\label{lem:funct-susp-commute}
  Given a group homomorphism $\phi : G_1 \to G_2$, we have $$\ap{\phi_{n+1}}{\sigma_n(x)} =_{\Omega(K(G_2,n))} \sigma_n(\phi_n(x))$$ for $x : K(G_1,n)$.
\end{lemma}

\subsection{Group structure}
\label{sec:emgroupstructure}

One of the key contributions of \cite{BLM} was the computationally
optimised definition of the h-space structure on
$K(\bZ,n) := \truncT{\mathbb{S}^n}_n$ (when $n \geq 1$). Our goal here
is to rephrase this optimised construction to $K(G,n)$ defined as
above.

\begin{proposition}
  \label{prop:wedgeconn}
  Let $n,m\geq 1$ and assume we are
  given a fibration $\widetilde{K}(G_1,n) \times
  \widetilde{K}(G_2,m) \to \ntype{(n+m-2)}$, sections $f : (x :
  \widetilde{K}(G_1,n)) \to P(x,\KO)$ and $g : (y : \widetilde{K}(G_2,m))
  \to P(\KO,y)$ and a path $p : f(0_k) = g(0_k)$.
%%   making both top triangles and the outer square in the
%%   following diagram commute:
%% \[\begin{tikzcd}[ampersand replacement=\&]
%% 	\&\& \underset{(x,y) : \widetilde{K}(G_1,n) \times \widetilde{K}(G_2,m)}{\sum} \!\!\!\!\!\!\!\!\!\! P(x,y) \\
%% 	{\widetilde{K}(G_1,n)} \&\& {\widetilde{K}(G_1,n) \times \widetilde{K}(G_2,m)} \&\& {\widetilde{K}(G_2,m)} \\
%% 	\&\& {\mathbbm{1}}
%% 	\arrow["{(-\,,0_k,\,f(-))}", from=2-1, to=1-3]
%% 	\arrow["{(-,0_k)}"{pos=0.6}, from=2-1, to=2-3]
%% 	\arrow["{(0_k,-,\,g(-))}"', from=2-5, to=1-3]
%% 	\arrow["{(0_k,-)}"'{pos=0.6}, from=2-5, to=2-3]
%% 	\arrow[from=1-3, to=2-3]
%% 	\arrow["{x\mapsto 0_k}",from=3-3, to=2-1]
%% 	\arrow["{x\mapsto 0_k}"', from=3-3, to=2-5]
%% \end{tikzcd}\]
In this case, there is a unique section $$\timeswedge{f}{g} : ((x , y)
: {\widetilde{K}(G_1,n) \times \widetilde{K}(G_2,m)}) \to P(x,y)$$ equipped with homotopies
\begin{align*}
  &l : (x : \widetilde{K}(G_1,n)) \to
  (\timeswedge{f}{g})(x,0_k) = f(x) \\
  &r : (y : \widetilde{K}(G_2,m))
  \to (\timeswedge{f}{g})(0_k,y) = g(y)
\end{align*}
satisfying $l(0_k)^{-1} \cdot r(0_k) = q$
\end{proposition}
\begin{proof}
  \anders{Kolla resten sen när eventuella typos fixats (speciellt
    slutet)} An easy way of proving the above lemma is to note that
  the canonical map $i_{\vee} : {\widetilde{K}(G_1,n) \vee
    \widetilde{K}(G_2,m)} \to {\widetilde{K}(G_1,n) \times
    \widetilde{K}(G_2,m)}$ is $(n-1) + (m-1)$-connected, thereby
  inducing a section via the map $f \vee g : (x :
  {\widetilde{K}(G_1,n) \vee \widetilde{K}(G_1,m)}) \to P
  (i_\vee(x))$. From the point of view of computer formaisation,
  however, this proof leads to poor computational behvaiour of
  subsequent definitions. For this reason, we provide a direct proof.

  We proceed by induction on $n$ and $m$. We first consider the
  base-case: $n=m=1$. We are to construct a section $\timeswedge{f}{g}
  : ((x,y): \widetilde{K}(G_1,1) \times \widetilde{K}(G_2,1)) \to
  P(x,y)$. Since $P$ is a set, it suffices to define a section
  $\timeswedge{f}{g} : ((x,y): L(G_1) \times L(G_2)) \to P(x,y)$. Let $q:
  f(\KO) = g(\KO)$. We proceed by $L(G_1)$-induction on $x$. For the point constructor, we define
  \begin{align*}
    (\timeswedge{f}{g})(\star,y) &:= g(y)
  \end{align*}
  We now need to define $\ap{(\timeswedge{f}{g})(-,y)}{\LoopG{a}}$ for $a : G_1$. Since $P$ is set valued, it suffices to do so when $y$ is $\star$. We define
  \begin{align*}
    \ap{(\timeswedge{f}{g})(-,\star)}{\LoopG{a}} &:= q^{-1}\cdot \ap{f}{\LoopG{a}} \cdot q
  \end{align*}
We note that this
construction satisfies the additional properties by default: we
construct $l : (x : \widetilde{K}(G_1,1)) \to (\timeswedge{f}{g})(x,\KO)
= f(x)$ by induction on $x$. Since this is a proposition, it suffices
to construct $l(0_k) : g(\KO) = f(\KO)$, which we do by $l(0_k) :=
q^{-1}$. We construct $r : (y : \widetilde{K}(G_2,1)) \to
(\timeswedge{f}{g})(\KO,x)$ simply by $r(y) := \refl$, since the
equality holds by definition. We finally need to show that ${l(0_k)}^{-1}
\cdot r(0_k)= q$ which is immediate by construction of $l$ and $r$.

We proceed by induction on $n$, letting $n \geq 2$ and omitting the case $(1,m)$ which is
completely analoguous. We define $\timeswedge{f}{g} : ((x , y) :
{\widetilde{K}(G_1,n) \times \widetilde{K}(G_2,m)}) \to P(x,y)$. We stress that since
$n \geq 2$, we have that $\widetilde{K}(G_1,n) = \Sigma
\widetilde{K}(G_1,n-1)$ by definition. Hence, we may define
$\timeswedge{f}{g}$ by suspension induction on $x$. We start with the
action on point constructors.
\begin{align*}
  (\timeswedge{f}{g})(\mathsf{north},y) &:= g(y)\\
  (\timeswedge{f}{g})(\mathsf{south},y) &:= \transport{P(-,y)}{\merid{\KO}}{g(y)}
\end{align*}
We finally need to define $\ap{\timeswedge{f}{g}}{-,y}(\merid{a}) :
\Square{g(y)}{\transport{P(-,y)}{\merid{\KO}}{g(y)}}{P(-,y)}{\merid{a}}$
for $a :\widetilde{K}(G_1,n-1)$ and $y : \widetilde{K}(G_2,m)$. The type
of $\ap{\timeswedge{f}{g}}{-,y}(\merid{a})$ is an $(n+m-3)$-type, and
thus, by induction hypothesis, it suffices to construct the following:
\begin{align*}
  f' &: (a : \widetilde{K}(G_1,n-1))\to\Square{g(\KO)}{\transport{P(-,\KO)}{\merid{\KO}}{g(\KO)}}{P(-,\KO)}{\merid{a}} \\
  g' &: (y : \widetilde{K}(G_2,m))\to \Square{g(y)}{\transport{P(-,y)}{\merid{\KO}}{g(y)}}{P(-,y)}{\merid{\KO}} \\
  q' &: f'(\KO) = g'(\KO)
\end{align*}
%
By composition with $q$, the target type of $f'$ is equivalent to the
type $\Square{f(\north)}{f(\south)}{P(-,\KO)}{\merid{a}}$, of which we
have a term: $\ap{f}{\merid{a}}$. The target type of $g'$ is
equivalent to $g(y) = g(y)$. We simply give the term $\refl$. Showing
that $q'$ holds is an easy but technical lemma. Thus we have
constructed $\timeswedge{f}{g}$. Note now that $r : (y :
\widetilde{K}(G_2,m)) \to (\timeswedge{f}{g})(\KO,y) = g(y)$ holds by
$\refl$. The path $l : (x : \widetilde{K}(G_1,n-1)) \to
(\timeswedge{f}{g})(x,\KO) = g(y)$ is easily shown using the
correponding $l$- and $r$-paths from the inductive hypothesis. This
can be done in a way such that the fact that $l(\KO) = r(\KO)$ holds
almost by definition.
\end{proof}

Our goal is now to define addition $+_k : K(G,n) \times K(G,n) \to
K(G,n)$. When $n = 0$, it is simply addition in $G$. For $n \geq 1$,
we note that, by the elimination principle
for $K(G,n)$ in Figure~\ref{elim:KG}, it suffices
to define a corresponding operation $+_k : \widetilde{K}(G,n) \times
\widetilde{K}(G,n) \to K(G,n)$.
When $n = 1$, we define it explicitly by
\begin{align*}
  \star +_k y &:= y\\
  \ap{\_ +_k \star}{\LoopG{g}}  &:= \LoopG{g} \\
  \ap{\lambda x \, \to \ap{\_ +_k x}{\LoopG{g_1}}} {\LoopG{g_2}}  &:= Q
\end{align*}
where $Q$ is a filler of the following square
\[\begin{tikzcd}[ampersand replacement=\&]
	\star \& \star \\
	\star \& \star
	\arrow["{\LoopG{g_1}}", from=1-1, to=1-2]
	\arrow["{\LoopG{g_1}}"', from=2-1, to=2-2]
	\arrow["{\LoopG{g_2}}"', from=2-2, to=1-2]
	\arrow["{\LoopG{g_2}}", from=2-1, to=1-1]
\end{tikzcd}\]
which is easily constructed using that $\LoopG{}$ preserves composition
by definition of $K(G,n)$. All other cases are immediate since
$K(G,n)$ is $1$-truncated. For higher values of $n$, the construction
is made straightforward by Proposition~\ref{prop:wedgeconn}. We have
that $K(G,n)$ is $(n-1)$-connected and is of truncation level $n\leq
2(n-1)-2$. That latter inequality holds precisely when $n \geq
2$. Therefore, we may define $+_k$ simply by
\begin{align}
  \label{eq1}
  x +_k 0_k & := x \\
  \label{eq2}
  0_k +_k y & := y
\end{align}
Proposition \ref{prop:wedgeconn} also requires us to prove the above
definitions to coincide when $x= 0_k$ and $y = 0_k$, which they do by
$\refl$. Thus we have defined $+_k : \widetilde{K}(G,n) \times
\widetilde{K}(G,n) \to K(G,n)$, which lifts to an addition $K(G,n)
\times K(G,n) \to K(G,n)$ which we, abusing notation, will also denote
by $+_k$.

The laws governing $+_k$ are remarkably easy to prove.
\begin{proposition}
  \label{prop:+-unit}
  The addition $+_k$ has $0_k$ as a left- and-
  right-unit. Furthermore, these are coherent in the sense that we
  have a filler of the following square \textnormal{
    \[\begin{tikzcd}[ampersand replacement=\&]
	{0_k + 0_k} \& {0_k} \\
	{0_k + 0_k} \& {0_k}
	\arrow["{\textsf{r-unit}}(0_k)", from=1-1, to=1-2]
	\arrow[Rightarrow, no head, from=1-1, to=2-1]
	\arrow["{\textsf{l-unit}}(0_k)"', from=2-1, to=2-2]
	\arrow[Rightarrow, no head, from=1-2, to=2-2]
\end{tikzcd}\]}
\end{proposition}
\begin{proof}
  The statement follows from the group structure on $G$ when $n =
  0$. When $n = 1$ the target type is a set, since $K(G,1)$ is
  $1$-truncated (and hence path types over it are sets). By the
  set-elimination rule for $K(G,n)$ (see~Figure~\ref{elim:KG-set}) it
  suffices to show that $\trunc{x} +_k 0_k = 0_k = 0_k +_k \trunc{x}$
  for $x : L(G)$. These equalities hold definitionally by $L(G)$
  induction. Hence, we also get the filler of the square by
  $\refl$. When $n \geq 2$, the statement follows immediately by the
  defining equations~\eqref{eq1}~and~\eqref{eq2}, using the family of
  paths $l$ and $r$ and the coherence between them, as given in
  Proposition \ref{prop:wedgeconn}.
\end{proof}

In fact, modulo $\mathbb{N}$-induction, by the direct proof of
Proposition \ref{prop:wedgeconn}, we get that the left-and right-unit
laws are definitionally equal at $0_k$, with both definionally equal
to $\refl$.

\begin{proposition}
  \label{prop:+-comm}
  The addition $+_k$ is commutative.
\end{proposition}
\begin{proof}
  When $n = 0$, the statement is simply that $G$ is abelian, which we
  have assumed.  Let $n \geq 1$.  By truncation elimination, it
  suffices to construct paths $\trunc{x} +_k \trunc{y} = \trunc{y} +_k
  \trunc{x}$ for $x,y:\widetilde{K}(G,n)$. This path type is
  $(n-1)$-truncated which is sufficiently low for Proposition
  \ref{prop:wedgeconn} to apply. Hence it suffices to construct paths
  $p_x : \trunc{x} + 0_k = 0_k + \trunc{x}$ and $q_y : 0_k +_k
  \trunc{y} = \trunc{y} + 0_k$ and show that $p_{0_k} = q_{0_k}$. We
  construct both paths as compositions of the left- and right-unit
  laws of $+_k$ in the obvious way. These definitions coincide over
  $0_k$ by the square in Proposition \ref{prop:+-unit}.
\end{proof}

The following proposition is equally direct to prove, so we omit its
proof.
%
\begin{proposition}
  \label{prop:+-assoc}
  The addition $+_k$ is associative.
\end{proposition}
%
Propositions~\ref{prop:+-unit},~\ref{prop:+-comm}~and~\ref{prop:+-assoc}
amount precisely to showing that $K(G,n)$ is a commutative,
associative h-space. There is, however, more to the story. In HoTT, it
is easy to define an inversion on $K(G,n)$. When $n = 0$, it is simply
negation in $G$. When $n \geq 1$, we have two different options. One
approach is to note that for any $x : K(G,n)$, the map
$y \mapsto x + y$ is an equivalence. This is
proved by observing that the property of being an equivalence is a
proposition. The elimination rule of $K(G,n)$ into $(n-2)$-types tells
us that it is enough to show that the map is an equivalence when $x$
is $0_k$; in this case the map is simply the identity, and thus also
an equivalence. The unique element in the fibre of $y \mapsto x + y$
over $0_k$ is taken to be the inverse of $x$. This proof also gives
the desired cancellations laws by construction. This is the approach
used in e.g.\ \citep{Brunerie16,LicataFinster14}.

While elegant, the above approach has one major disadvantage: the
action of $-_k$ on any element other than $0_k$ is described using
transports. One consequence of this is that the terms produced by
$-_k$ often are hard to work with directly. Another consequence is
that terms decscribed using $-_k$ tend to explode in size, which leads
to poor computatonal behaviour in implementations in proof
assistants. For these reasons, we choose the obvious direct
construction of $-_k$. We define it as a map
$-_k : \widetilde{K}(G,n) \to \widetilde{K}(G,n)$. When $n = 1$, we
define
\begin{align*}
  -_k \,\star &:= \star\\
  \ap{-_k}{\LoopG{g}} &:= (\LoopG{g})^{-1}\\
  \ap{\mathsf{ap}_{-_k}}{\mathsf{sq}\,g_1\,g_2} &:= Q
\end{align*}
where $Q$ is a filler of the square
\[\begin{tikzcd}[ampersand replacement=\&]
	\star \&\& \star \\
	\star \&\& \star
	\arrow[Rightarrow, no head, from=2-1, to=1-1]
	\arrow["{(\LoopG{g_1})^{-1}}"', from=2-1, to=2-3]
	\arrow["{\LoopG{(g_1+g_2)}^{-1}}", no head, from=1-1, to=1-3]
	\arrow["{(\LoopG{g_2})^{-1}}"', from=2-3, to=1-3]
\end{tikzcd}\]
which is easy to construct using the functoriality of $\LoopG{}$.
For $n \geq 2$, we define it by
\begin{align*}
  -_k \, \north &:= \north\\
  -_k \, \south &:= \north\\
  \ap{-_k}{\merid{g}} &:= \sigma_n(g)^{-1}
\end{align*}

For the cancellation laws, we will need the following lemma. We remark
that it is only is well-typed in the case when $n = 1$ is fixed or
when $n$ is on the form $(2 + m)$.
The fact that it is well-typed exploits the fact that
$0_k = 0_k +_k 0_k$ holds definitionally modulo the case distinction
on $n$.
\begin{proposition}
  \label{prop:ap-+}
  Let $n \geq 1$. Given $p, q : \Omega (K(G,n))$, we have
  $\app{+_k}{p}{q} = p \cdot q$.
\end{proposition}
\begin{proof}
  We have
  \[
\app{+_k}{p}{q} = \ap{x\mapsto x +_k 0_k}{p} \cdot \ap{y\mapsto 0_k +_k y}{q} = p \cdot q
\]
The final step consists in applying the right- and left-unit laws to
both components. This is justified since they agree at $0_k$.
\end{proof}

We write $x -_k y$ for $x +_k (-_k\,y)$ and have that the directly
defined $-_k$ is indeed inverse to $+_k$ by:

\begin{proposition}
  For $x : K(G,n)$, we have $x -_k x = 0_k = (-_k\,x) +_k x$.
\end{proposition}
\begin{proof}
  By commutativity of $+_k$, it it suffices to show that
  $x -_k x = 0_k$. When $n = 0$, this comes from the group structure
  on $G$. When $n = 1$, we note that the goal type is a set, which
  means that it suffices to show the statement for $x : L(G)$. We have
  $\star -_k \star = 0_k$ by $\refl$. For $\LoopG{}$, we need to show
  that
    \[
    \app{x,y\mapsto x -_k y}{\LoopG{g}}{\LoopG{g}} = \refl
    \]
    By functoriality of $\mathsf{ap}^2$
    and the unit laws for $+_k$, the LHS above is equal to
    $\LoopG{g} \cdot (\LoopG{g})^{-1}$ which is equal to $\refl$. The
    case when $n \geq 2$, is entirely analoguous, using~Proposition~\ref{prop:ap-+} for the path constructors.
\end{proof}

And there we have it: the $3$-tuple $(K(G,n),+_k,0_k)$ forms, for any
$n$, a commutative h-space with inverse given by $-_k$. We will in
Section~\ref{sec:cohomology} see that this trivially gives an induced
group structure on cohomology groups, but first we will look closer at
$\sigma_n$ and then consider the multiplicative structure on $K(G,n)$.

\subsection{$K(G,n)$ vs. $\Omega K(G,n+1)$}
\label{sec:omegakgn}

We will soon see that $\sigma_n : K(G,n) \to \Omega K(G,n+1)$ is in
fact an equivalence. This equivalence will be crucial when computing
cohomology groups of spaces. However, we do not need it yet:
Proposition~\ref{prop:ap-+} already provides us with a strong link
between the structures on $K(G,n)$ and $\Omega K(G,n+1)$. For
instance, we may already now deduce the commutativity of
$\Omega K(G,n+1)$ from the commutativity of $+_k$:
\begin{proposition}
  \label{prop:comm-path}
  For $x : K(G,n)$ and $p,q : x = x$, we have $p \cdot q = q \cdot p$.
\end{proposition}
\begin{proof}
  When $n = 0$, we are automatically done, since $G$ is a set. For
  $n \geq 1$, it suffices, by $(n-2)$-type elimination, to show the
  statement when $x$ is $0_k$. Let $p,q: \Omega K(G,n)$. We have
  \begin{align*}
    p \cdot q = \app{+_k}{p}{q} = \app{+_k}{q}{p} = q \cdot p
  \end{align*}
  where the second equality comes from the commutativity of $+_k$.
\end{proof}

The usefulness of the above proof (as opposed to one using an
equivalence $K(G,n) \simeq \Omega K(G,n+1)$ as in~\cite{Brunerie16})
is that it is rather direct and is easily shown to be homotopically
trivial when $p$ and $q$ are $\refl$.

On a similar note, we may also provide a direct proof of the following proposition.
%
\begin{proposition}
  \label{prop:ap--}
  Let $n \geq 1$ and $p: \Omega K(G,n)$, we have $\ap{-_k}{p} = p^{-1}$.
\end{proposition}
\begin{proof}
  \anders{Dubbelkolla det här beviset igen när eventuella typos är fixade}
  We provide the proof for $n = 1$. The case when $n > 1$ is entirely
  analoguous. We will employ the encode-decode method. We define
  $\mathsf{Code}_x: (p : \star = x) \to \mathsf{hProp}$ for
  $x:K(G,1)$. As $\mathsf{hProp}$ is a $0$-type, it suffices to define
  $\mathsf{Code}_x(p)$ where $x : L(G)$. We do this by induction on
  $x$ and define
  \begin{align*}
    \mathsf{Code}_\star(p) := (\ap{-_k}{p} = p^{-1})
  \end{align*}
  which is a proposition since $K(G,1)$ is $0$-connected. We need to
  check that this definition respects the action of $\mathsf{Code}$ on
  $\LoopG{g}$ for $g:G$. This amounts to showing that, for any $p :
  \Omega K(G,1)$, we have an equivalence
  \begin{align*}
    (\ap{-_k}{p} = p^{-1}) \simeq (\ap{-_k}{p \cdot \LoopG{g}} &= (p \cdot \LoopG{g})^{-1})
  \end{align*}
  We rewrite the terms on the RHS as follows:
  Using the following two rewritings on the RHS. We have
  \begin{align*}
    \ap{-_k}{p \cdot \LoopG{g}} &= \ap{-_k}{p} \cdot  \ap{-_k}{\LoopG{g}}
    \\ &= \ap{-_k}{p} \cdot {(\LoopG{g})}^{-1}
  \end{align*}
  and
  \begin{align*}
(p \cdot \LoopG{g})^{-1} &= (\LoopG{g})^{-1} \cdot p^{-1} \\
&= p^{-1} \cdot (\LoopG{g})^{-1}
  \end{align*}
Thus, we only need to construct an equivalence.
  \begin{align*}
    (\ap{-_k}{p} = p^{-1}) \simeq (\ap{-_k}{p} \cdot (\LoopG{g})^{-1} &= p^{-1} \cdot (\LoopG{g})^{-1})
  \end{align*}
  This equivalence is given by $\mathsf{ap}_{q \mapsto q \cdot
    (\LoopG{g})^{-1}}$ and thereby the construction of $\mathsf{Code}$
  is complete.

  We now note, as usual, that we have a section
  $(p : \star = x) \to \mathsf{Code}_x(p)$ for any $x:K(G,1)$ by path
  induction, it suffices to note that $\refl_\star$ is an element of
  $\mathsf{Code}_\star(\refl)$. Hence, in particular, we have an
  element of $\mathsf{Code}_\star(p)$ for all $p : \Omega K(G,1)$,
  which is what we wanted to show.
\end{proof}

The following proposition is
  also crucial and its proof can be found in
  \citet[Lemma~4.4]{LicataFinster14}.
\begin{proposition}
  \label{prop:+-hom}
  For $x,y : K(G,n)$, we have $\sigma_n(x +_k y) = \sigma_n(x) \cdot
  \sigma_n(y)$.
\end{proposition}
% \begin{proof}
%   \anders{Dubbelkolla detaljerna och korrläs}
%   \todo{maybe omit and just refer to FinsterLicata} When $n = 0$, we
%   need to show that $\LoopG{(x + y)} = \LoopG{x} \,\cdot \LoopG{y}$, which
%   holds by definition of $K(G,1)$. For $n \geq 1$,
%   Proposition \ref{prop:wedgeconn} applies, and it suffices to provide paths
%   $\sigma_n(0_k +_k y) = \sigma_n(0_k)\cdot\sigma_n(y)$ and $\sigma_n(x +_k
%   0_k) = \sigma_n(x)\cdot\sigma_n(0_k)$ and show that these coincide when
%   $x$ and $y$ are $0_k$. This is easy but somewhat technical, so we
%   omit the proof and refer to the original proof by~\cite[Lemma 2]{LicataFinster14}.
% \end{proof}

Because $\sigma_n$ is pointed, Proposition~\ref{prop:+-hom}
immediately gives us the following corollary (which is proved just
like in group theory).
\begin{corollary}
  \label{prop:--hom}
  For $x: K(G,n)$, we have $\sigma_n(-_k \, x) = \sigma_n(x)^{-1}$.
\end{corollary}
%
%% Another more direct connection between the $K(G,n)$ and $\Omega
%% K(G,n)$ is given by the following proposition.
%% We also arrive at a similar conclusion for the action of
%% $\mathsf{ap}_{-_k}$.
We are now ready for the main result of the section, namely that
$\Omega K(G,n+1) \simeq K(G,n)$. The original proof in HoTT is due
to~\cite[Theorem 4.3]{LicataFinster14} who used encode-decode proofs
in the cases $n=0$ and $n=1$, and the Freudenthal suspension theorem
(formalised in HoTT by~\cite{FavoniaFinster+16}) in the case $n \geq
2$. Here we use an identical proof in the case $n = 1$. However, it is
possible to avoid the Freudenthal suspension theorem completely by
simply noting that the proof of Licata~and~Finster when $n = 1$
actually can be used for all $n \geq 1$. We primarily wish to avoid
the Freudenthal suspension theorem as circumventing it makes the
computer formalisation more computationally viable. We will discuss
this further in Section~\ref{sec:computations}.
%
\begin{theorem}
  \label{thm:deloop}
  The map $\sigma_n : K(G,n) \to \Omega K(G,n+1)$ is an equivalence.
\end{theorem}
\begin{proof}
  For $n = 0$, we refer to the proof in~\cite{LicataFinster14}. For
  $n \geq 1$, we choose to provide an encode-decode proof similar to
  their $n = 1$ case. We define
  $\mathsf{Code} : K(G,n+1) \to \ntype{n}$ by
\begin{align*}
  \mathsf{Code}(\trunc{\north}) &:= K(G,n) \\
  \mathsf{Code}(\trunc{\south}) &:= K(G,n) \\
  \ap{\mathsf{Code}\,\circ\, \trunc{-}}{\merid\,a} &:= \mathsf{ua}(x \mapsto \trunc{a} +_k x)
\end{align*}
%\anders{Är inte ``univalence'' bara ``ua''? Vi borde introducera vår notation för de olika delarna i univalence i bakgrunden. Sen är det väl inte riktigt bara funktionen utan ekvivalensen...
%Tänkte att det här blev väldigt tydligt, så slipper man introducera notation...
% }
Here $\mathsf{ua}$ is the part of univalence which turns an equivalence into a path. Clearly the map to which it is applied is an equivalence.
For any $t : K(G,n+1)$, we have a map $\mathsf{encode}_t : 0_k = t \to
\mathsf{Code}(t)$ defined by
$\mathsf{encode}_t(p):=\transport{\mathsf{Code}}{p}{0_k}$ (this is
equivalent to path induction on $p$). We define $\mathsf{decode}_t :
\mathsf{Code}(t) \to 0_k = t$ by truncation elimination and
$K(G,n)$-induction on $t$. For the point constructors, we define it by
\begin{align*}
  \mathsf{decode}_{\trunc{\north}}(x) &= \sigma_n(x)\\
  \mathsf{decode}_{\trunc{\south}}(x) &= \sigma_n(x)\cdot \ap{\trunc{-}}{\merid{0_k}}
\end{align*}
For the path constructor, we need to, after some simple rewriting of the goal, provide a path
\[
\sigma_n(x-_k\trunc{a}) = \sigma_n(x)\cdot \sigma_n(\trunc{a})^{-1}
\]
for $x : K(G,n)$ and $a : \widetilde{K}(G,n)$ which is easily done using Proposition~\ref{prop:+-hom} and Corollary~\ref{prop:--hom}. We can now show that, for any $t : K(G,n+1)$ and $p
: 0_k = t$, we have $\mathsf{encode}_t(\mathsf{decode}_t(p)) = p$ by
path induction on $p$. In particular, we have
$\mathsf{decode}_{0_k}(\mathsf{encode}_{0_k}(p)) = p$ for all $p :
\Omega K(G,n+1)$. We can also show that
$\mathsf{encode}_{0_k}(\mathsf{decode}_{0_k}(x)) = x$ for all
$x:K(G,n)$ by simply unfolding the definitions of
$\mathsf{decode}_{0_k}$ and $\mathsf{encode}_{0_k}$. Indeed, after applying truncation elimination on $x$, we have:
\begin{align*}
  \mathsf{encode}_{0_k}(\mathsf{decode}_{0_k}(\trunc{a})) &:= \mathsf{encode}_{0_k}(\sigma_n(\trunc{a})) \\
  &:= \transport{\mathsf{Code}}{\sigma_n(\trunc{a})}{0_k}\\
  &= \transport{\mathsf{Code}\circ \trunc{-}}{\merid(0_k)^{-1}}{\transport{\mathsf{Code}\circ \trunc{-}}{\merid{a}}{0_k}} \\
  &= \transport{\mathsf{Code}\circ \trunc{-}}{\merid(0_k)^{-1}}{\trunc{a}+0_k}\\
  &=(-_k 0_k) +_k (\trunc{a}+0_k)\\
  &= \trunc{a}
\end{align*}
and we are done.
\end{proof}

Note that this implies that we have $\Omega^n (K(G,n)) \simeq G$. By
Proposition~\ref{prop:+-hom}, this equivalence is an isomorphism of
groups. Together with Proposition~\ref{prop:K-connected}, this shows
that $K(G,n)$ indeed is an Eilenberg-MacLane space.

\subsection{The cup product with group coefficients}
\label{sec:cupprodgroupcoeff}

There is an additional structure definable already on
Eilenberg-MacLane spaces: the cup product. The cup product has been
developed in HoTT before: the first construction was
in~\citet{Brunerie16}, where he defines
$\smile_k \, : K(\bZ,n) \times K(\bZ,m) \to K(\bZ,n+m)$. This
definition was later extended to a cup product
$\smile_k \, : K(G_1,n) \times K(G_2,m) \to K(G_1 \otimes G_2,n+m)$ by
\citet{Baumann18}. The issue with the definition of these cup products
is that they rely heavily on the properties of smash products. As a
consequence, not all cup product axioms have been formally verified
using these definitions. For this reason, a new definition of the cup
product on $\bZ$-cohomology was given by~\citet{BLM}, which allowed
for a complete proof of the graded commutative ring laws. Our goal in
this section is to generalize this definition to a map
$\smile_k \, : K(G_1,n) \times K(G_2,m) \to K(G_1 \otimes G_2,n+m)$
which, like the definition by~\cite{BLM} avoids smash products, and
show that it satisfies the expected laws.

Before defining the cup product, we need to define tensor products of
abelian groups. In HoTT, we can do this very directly using the
obvious HIT.
%
\begin{definition}
  Given abelian groups $G_1$ and $G_2$ we define their tensor product
  $G_1 \otimes G_2$ by
  \begin{itemize}
    \item Points $g_1 \otimes g_2 : G_1 \otimes G_2$, for each $g_1 :G_1$ and $g_2:G_2$
    \item Points $\plustimes{x}{y}$ for each pair of points $x,y : G_1 \otimes G_2$
    \item For any $x,y,z : G_1 \otimes G_2$ paths
      \begin{align*}
        \plustimes{x}{y} &= \plustimes{y}{x} \\
        \plustimes{x}{(\plustimes{y}{z})} &= \plustimes{(\plustimes{x}{y})}{z} \\
        \plustimes{(0_{G_1} \otimes 0_{G_1})}{x} &= x
      \end{align*}
    \item For any $x : G_1$ and $y,z : G_2$,
      paths $x \otimes (y +_{G_2} z) = \plustimes{(x \otimes y)}{(x \otimes z)}$
    \item For any $x, y : G_1$ and $z : G_2$,
      paths $(x +_{G_1} y) \otimes z = \plustimes{(x \otimes z)}{(y \otimes z)}$
    \item A constructor $\normalfont{\textsf{is-set} : \mathsf{isSet}\,(G_1 \otimes G_2)}$
  \end{itemize}
\end{definition}
One easily verifies that this construction has the expected universal
property. Consequently, a map out of $G_1 \otimes G_2$ into a set is
defined if it is structure preserving. When mapping into a
proposition, it suffices to construct the map over canonical elements
$g_1 \otimes g_2$ and show that the proposition respects $\oplus$.

Let us return to the problem at hand: defining the cup product. We
note first that it is very easy to define a preliminary cup product
\begin{align}
  \label{red-cup}
  {\smile}_k' : \widetilde{K}(G_1,n) \times K(G_2,m) \to K(G_1 \otimes G_2,n+m)
\end{align}

When $n = 0$, we define $g \smile_k' (-)$ by the functorial action of $K(-,m)$ on the group homomorphism given by $g \otimes (-) : G_2 \to G_1 \otimes G_2$. When $n = 1$, we inductively define
\begin{align*}
  \star \smile_k' y &:= 0_k\\
  \ap{x \mapsto x \smile_k'\,y}{\LoopG{g}} &:= \sigma_m(x \smile_k' y)
\end{align*}
The fact that this respects the $\mathsf{sq}$ constructor is easy to
check. For $n \geq 2$, the idea is the same
\begin{align*}
  \north \smile_k' y &= 0_k\\
  \south \smile_k' y &= 0_k\\
  \ap{x \mapsto x \smile_k'\,y}{\merid\,a} &= \sigma_{(n-1)+m}(a \smile_k' y)
\end{align*}
We would now like to be able to lift $\smile_k'$ to a full cup product
$\smile_k \, : K(G_1,n) \times K(G_2,m) \to K(G_1 \otimes G_2,n+m)$:
\[\begin{tikzcd}[ampersand replacement=\&]
	{\widetilde{K}(G_1,n) \times K(G_2,m)} \& {K(G_1\otimes G_2,n+m)} \\
	{K(G_1,n) \times (K(G_2,m)}
	\arrow["{\smile_k'}", from=1-1, to=1-2]
	\arrow[from=1-1, to=2-1]
	\arrow[dotted, from=2-1, to=1-2]
\end{tikzcd}\]
or, after currying:
\[\begin{tikzcd}[ampersand replacement=\&]
	{\widetilde{K}(G_1,n)} \& {(K(G_2,m) \to K(G_1\otimes G_2,n+m))} \\
	{K(G_1,n)}
	\arrow["{\smile_k'}", from=1-1, to=1-2]
	\arrow[from=1-1, to=2-1]
	\arrow[dotted, from=2-1, to=1-2]
\end{tikzcd}\]
However, we run into an obstruction: for this lift to
exist, we require the function type ${K(G_2,m) \to K(G_1\otimes G_2,n+m)}$ to be an
$n$-type, which it is not unless $m = 0$. Fortunately, a very trivial
observation makes the lift possible: we want our cup product to
satisfy $x \smile_k 0_k = 0_k$. In other words, we may instead see the
cup product as a map into a pointed function space:
\begin{align*}
  \smile_k \, : K(G_1,n) \to (K(G_2,m) \to_\star K(G_1 \otimes G_2,n+m))
\end{align*}
In this case, we do get a lift
\[\begin{tikzcd}[ampersand replacement=\&]
	{\widetilde{K}(G_1,n)} \& {(K(G_2,m) \to_\star K(G_1\otimes G_2,n+m))} \\
	{K(G_1,n)}
	\arrow["{\smile_k'}", from=1-1, to=1-2]
	\arrow[from=1-1, to=2-1]
	\arrow["{\smile_k}"', dotted, from=2-1, to=1-2]
\end{tikzcd}\]
and thereby the cup product is defined. The existence of the lift is
motivated by the following result which follows from a more general
result~\cite[Corollary 1]{BDR18}, but has a very simple direct proof
when the spaces involved are Eilenberg-MacLane spaces.

\begin{proposition}
  \label{prop:pointed-hlevel}
  The space $K(G_1,n) \to_\star K(G_2,n+m)$ is $m$-truncated.
\end{proposition}
\begin{proof}
  It is enough to show that $\Omega^{m+1}(K(G_1,n) \to_\star
  K(G_2,n+m))$ is contractible. We have
  \begin{align*}
    \Omega^{m+1} (K(G_1,n) \to_\star K(G_2,n+m)) &\simeq (K(G_1,n) \to_\star \Omega^{m+1} K(G_2,n+m)) \\
    &\simeq (K(G_1,n) \to_\star K(G_2,n-1))
  \end{align*}
  The fact that $(K(G_1,n) \to_\star K(G_2,n-1))$ is contractible
  follows easily from the the $(n-2)$- type elimination rule for
  $K(G_1,n)$ in Figure~\ref{elim:KG-triv}.
\end{proof}
This concludes the construction of $\smile_k$. Let us now prove the various ring laws governing it. We first note that since $\smile_k'$ is pointed in both arguments, this also applies to $\smile_k$. Thus, we have verified the first law:
\begin{proposition}
  For $x : K(G,n)$, we have $x \smile_k 0_k = 0_k$ and $0_k \smile_k x = 0_k$.
\end{proposition}
We now set out to prove the remaining laws.
This turns out to be rather difficult to do directly: we want to prove
these laws using $K(G,n)$-elimination via Proposition
\ref{prop:pointed-hlevel}. This forces us to prove equalities of
pointed maps, rather than just maps. For instance, for
left-distributivity we have to prove that for any two points
$x,y: K(G_1,n)$ we have that the two maps
\begin{align*}
  z &\mapsto (x +_k y) \smile_k z \\
  z &\mapsto (x \smile_k z) +_k (y \smile_k z)
\end{align*}
are equal as \emph{pointed} maps living in $K(G_2,m) \to_\star K(G_1
\otimes G_2 , n + m)$. This is far more involved than proving equality
of the underlying maps: a proof of equality of pointed maps
$(f,p),(g,q) : A \to_\star B$ consists not only of a homotopy $h : (a
: A) \to f\,a = g\,a$, but also
a coherence $\Square{p}{q}{h(\star_A)}{\refl}$. Fortunately, there is
a trick to automatically infer the coherence.  We attribute this
result to Evan Cavallo.\footnote{The original form of the lemma was
  conjectured only for Eilenberg-MacLane spaces and appears as
  \cite[Lemma~14]{BLM}. Its proof, and generalisation to arbitrary
  homogeneous types, is attributed to Cavallo
  \cite[Lemma~A.27]{BLM}. Cavallo's original formalisation can be
  found in~\cite{HomogeneousFormalization}. The result has later been generalised in~\cite[Lemma 2.7]{buchholtz2023central}}

\todo{Då vi inte använt homogeneous types tidigare, kanske borde vi
  introducera det här så att läsaren inte behöver gå tillbaka 15
  sidor?}

\begin{lemma}[Evan's trick]
  \label{lem:Evan}
  Given two pointed functions $(f,p), (g,q) : A \to_\star B$ with $B$ homogeneous.
  If $f = g$, then there is a path of pointed functions $(f,p) = (g,q)$.
\end{lemma}
\begin{proof}
  By assumption, we have a homotopy $h : (x : A) \to f(x) = g(x)$. We
  construct a loop
  \begin{align*}
    r &: \star_B = \star_B \\
    r &:= p^{-1} \cdot h(\star_A) \cdot q
  \end{align*}
  and define
  \begin{align*}
    P &: (B,\star_B) =_{\mathcal{U}_*} (B,\star_B) \\
    P &:= \ap{(B,-)}{r}
  \end{align*}
  We get $P = \refl$ as an easy consequence of the homogeneity of
  $B$. Hence, instead of proving that $(f,p) = (g,q)$, it is enough to
  prove that $\transport{{A \to_\star (-)}}{P}{(f,p)} = (g, q)$. The
  transport only acts on $p$ and $q$, so the identity of the first
  components holds by $h$. For the second components, we are reduced
  to proving that $p \cdot r = h(\star_A) \cdot q$. This is true
  immediately by the construction of $r$.
\end{proof}

\begin{proposition}[Left-distributivity of $\smile_k$]
  Let $x,y : K(G_1,n)$ and $z : K(G_2,m)$. We have
  \[
  (x +_k y) \smile_k z = x \smile_k z +_k y \smile_k z
  \]
\end{proposition}
\begin{proof}
  When $n = 0$, the result follows by a straightforward induction on
  $m$. When $n \geq 1$ we generalise and, for $x,y : K(G_1,n)$,
  consider the two functions
  \begin{align*}
  z &\mapsto (x +_k y) \smile_k z \\
  z &\mapsto (x \smile_k z) +_k (y \smile_k z)
  \end{align*}
  We claim that these are equal as \emph{pointed} functions living in
  $K(G_2,m) \to_\star K(G_1\otimes G_2 , n + m)$. By Proposition
  \ref{prop:pointed-hlevel} all equality types over $K(G_2,m) \to_\star
  K(G_1\otimes G_2 , n + m)$ are $(n-1)$-types.
  This allows us to apply truncation elimination and Proposition
  \ref{prop:wedgeconn}. In combination with Lemma \ref{lem:Evan}, it
  suffices to show construct, for each $z : K(G_2,m)$:
  \begin{align*}
    l(y) &: (0_k +_k \trunc{y}) \smile_k z = (0_k \smile_k z) +_k (\trunc{y} \smile_k z)  \\
    r(x) &: (\trunc{x} +_k 0_k) \smile_k z = (\trunc{x} \smile_k z) +_k (0_k \smile_k z) \\
    q &: l(0_k) = r(0_k)
  \end{align*}
  which is direct using the unit laws
  for $+_k$ and $\smile_k$. The obvious construction makes $q$ hold
  by $\refl$.
\end{proof}
Right-distributivity follows by an almost identical proof, so we omit
it.
\begin{proposition}[Right-distributivity of $\smile_k$]
  Let $x: K(G_1,n)$ and $y,z : K(G_2,m)$. We have
  \[
  x \smile_k (y +_k z) = x \smile_k y +_k x \smile_k z
  \]
\end{proposition}
Before moving on to associativity, we will need the following
lemma. As pointed out by~\citet{BLM}, this lemma also appears
in~\citep[Proposition 6.1.1]{Brunerie16} where it is used for the
construction of the Gysin sequence. Its proof relies on e.g.\ the
pentagon identity for smash products which at the time was not fully
proved in HoTT. In our setting, which like \citep{BLM} uses pointed
maps instead of smash products, it holds by construction.
\begin{lemma}
  \label{lem:ap-cup}
  For $x : K(G_1,n)$ and $y : K(G_2,m)$, we have
  $$\ap{x\mapsto x \smile_k y}{\sigma_n(x)} = \sigma_{n+m}(x \smile_k y)$$
\end{lemma}
\begin{proof}
  When $n = 0$, the statement holds by definition. Let us consider the
  case $n \geq 1$. The maps we are comparing are of type $K(G_1,n) \to K(G_2,m)
  \to_\star \Omega (K(G_1 \otimes G_2 , (n + 1) + m))$. The
  type $$K(G_2,m) \to_\star \underset{\simeq K(G_1\otimes
    G_2,n+m)}{\underbrace{\Omega (K(G_1 \otimes G_2 , (n + 1) + m))}}$$ is an
  $n$-type by Proposition~\ref{prop:pointed-hlevel}, and hence we may
  use $K(G,n)$-elimination on $x$. Hence, we want to construct an equality of pointed functions
  \[(y\mapsto \ap{x\mapsto x \smile_k y}{\sigma_n(a)}) = (y \mapsto \sigma_{n+m}(a \smile_k' y))\]
  for $a : \widetilde{K}(G,n)$. By Lemma~\ref{lem:Evan} it suffices to
  show this equality for underlying functions.
\end{proof}
With Lemma \ref{lem:ap-cup}, associativity is straightforward to prove. This follows trivially:
\begin{align*}
  \ap{x\mapsto x \smile_k y}{\sigma_n(a)} &:= \ap{x\mapsto \trunc{x} \smile_k y}{\merid{a} \cdot (\merid{0_k})^{-1}} \\
  &= \ap{x\mapsto \trunc{x} \smile_k y}{\merid{a}} \cdot (\ap{x\mapsto \trunc{x} \smile_k y}{\merid{0_k}})^{-1}  \\
  &:= \sigma_{n+m}(a \smile_k' y) \cdot \sigma_{n+m}(0_k \smile_k' y)^{-1}\\
  &= \sigma_{n+m}(a \smile_k' y)
\end{align*}
which is what we wanted to show.
\begin{proposition}
  The cup product is associative, i.e.\ the following diagram
  commutes:
\[\begin{tikzcd}[ampersand replacement=\&]
	{K(G_1,n)\times K(G_2,m) \times K(G_3,k)} \&\&\& {K(G_1\otimes (G_2 \otimes G_3),n+(m+k))} \\
	\&\&\& {K((G_1\otimes G_2) \otimes G_3,(n+m)+k)}
	\arrow["{x,y,z\mapsto x \smile_k (y \smile_k z)}", from=1-1, to=1-4]
	\arrow["{x,y,z\mapsto (x \smile_k y) \smile_k z}"', sloped, from=1-1, to=2-4]
	\arrow["\sim", sloped, from=2-4, to=1-4]
      \end{tikzcd}\]
\end{proposition}
\begin{proof}
  We induct on $n$. Let us first consider the inductive step and save the base case for last. To this end, let $n \geq 1$. We may consider the two functions we are comparing
  as doubly pointed functions of type
  \[K(G_1,n) \to (K(G_2,m) \to_\star (K(G_3,k) \to_\star K(G_1 \otimes (G_2 \otimes G_3) , n + m + k)))\]
  Applying an appropriate variant of Proposition
  \ref{prop:pointed-hlevel}, the codomain of the above function type is
  an $n$-type. When $x$ is a point constructor of $K(G_1,n)$, the
  diagram in the statement commutes by $\refl$. For the higher
  constructor ($\merid$ or $\LoopG{}$, depending on the value of $n$),
  we are done if we can show, for $x : K(G_1,n-1)$, that
  \begin{align*}
    \ap{x \mapsto x \smile_k (y \smile_k z)}{\sigma_{n-1}(x)} = \ap{x \mapsto \alpha_{n+m+k} ((x \smile_k y) \smile_k z)}{\sigma_{n-1}(x)}
  \end{align*}
   where $\alpha : (G_1 \otimes G_2) \otimes G_3 \simeq (G_1 \otimes
   (G_2 \otimes G_3)$ and, recall, $\alpha_{p} : K((G_1 \otimes G_2)
   \otimes G_3,p) \to K(G_1 \otimes (G_2 \otimes G_3),p)$ is the
   functorial action of $K(-,p)$ in $\alpha$. We have
  \begin{align*}
    \ap{x \mapsto x \smile_k (y \smile_k z)}{\sigma_{n-1}(x)} &=
    \sigma_{(n-1)+(m+k)}(x \smile_k (y \smile_k z)) & \text{ (Lemma~\ref{lem:ap-cup})} \\
    &= \sigma_{(n-1)+(m+k)}(\alpha_{(n-1)+(m+k)} ((x \smile_k y) \smile_k z)) & \text{ (ind. hyp.)} \\
    &= \ap{\alpha_{n+m+k}}{\sigma_{((n-1) + m)+k}((x \smile_k y) \smile_k z)} &\text{ (Lemma~\ref{lem:funct-susp-commute})} \\
    &= \ap{\alpha_{n+m+k}}{\ap{x \mapsto x \smile_k z}{\sigma_{((n-1) + m)}(x \smile_k y)}} &\text{ (Lemma~\ref{lem:ap-cup})} \\
    &= \ap{\alpha_{n+m+k}}{\ap{x \mapsto x \smile_k z}{{\ap{x \mapsto x \smile y}{\sigma_{(n-1)}(x)}}}} &\text{ (Lemma~\ref{lem:ap-cup})} \\
    &= \ap{x \mapsto \alpha_{n+m+k} ((x \smile_k y) \smile_k z)}{\sigma_{n-1}(x)}
  \end{align*}
  Let us return to the base case, i.e. the case $n = 0$. In this case,
  we fix $g_1 : G_1$ and instead consider the functions $y,z \mapsto
  g_1 \smile_k(y\smile_k z)$ and $y,z \mapsto (g_1 \smile_k y)\smile_k
  z$ to be of type $$K(G_2,m) \to K(G_3,k) \to_\star K(G_1\otimes
  (G_2 \otimes G_3) , m + k).$$ We induct on $m$. The inductive step
  follows in the same way as the indctive step above. For the base
  case, we fix $y$ to be $g_2 : G_2$ and are left to prove $g_1
  \smile_k (g_2 \smile_k z) = (g_1 \smile_k g_2) \smile_k z$ for $z :
  K(G_3,k)$. Again, this is follows by inuction on $k$. The base case
  is given by associativity of $G_1\otimes (G_2 \otimes G_3)$ and the
  inductive step follows in exactly the same way as before.
\end{proof}
\begin{proposition}
  \label{prop:cup-comm}
  The cup product is graded commutative, i.e.\ the following diagram
  commutes:
\[\begin{tikzcd}[ampersand replacement=\&]
	{K(G_1,n)\times K(G_2,m)} \&\&\& {K(G_1\otimes G_2,n+m)} \\
	\&\&\& {K(G_2\otimes G_1,m+n)}
	\arrow["{x,y\hspace{1mm}\mapsto (-1)^{nm}(y \smile_k x)}"', sloped, from=1-1, to=2-4]
	\arrow["\smile_k", from=1-1, to=1-4]
	\arrow["\sim", sloped, from=2-4, to=1-4]
\end{tikzcd}\]
\end{proposition}
\begin{proof}
  We may, without loss of generality, assume that $n \geq m$. We
  induct on the quantity $n+m$. The base-case when $n = m = 0$ is
  trivial. Let us consider the two cases $n = m = 1$ and $n,m \geq 2$
  and omit the two cases when $n \geq 2$ and $m < 2$ -- they
  follows in an entirely analogous manner. In what follows, let $c_p :
  K(G_2\otimes G_1,p) \to K(G_1 \otimes G_2,p)$ denote the commutator.

We start with the case $n = m = 1$. In this case, we would like to be
able to apply the set-elimination rule for $K(-,1)$. As before, fix $x
: K(G_1,1)$. We strengthen the goal by asking for $x \smile_k (-)$ and
$y \mapsto (-1)^{nm}(y \smile_k x)$ to be equal as pointed functions
living in $K(G_2,1) \to_\star K(G_1\otimes G_2 , 2)$. The type of such
functions is a $1$-type, and hence any path type over it is a
set. Thus, we may apply set-elimination and assume that $x :
L(G_1)$. We may now repeat the argument for $y : K(G_2,n)$: we would
like $(-) \smile_k y$ and $x \mapsto (-1)^{nm}(y \smile_k x)$ to be equal
as pointed functions living in $L(G_1) \to_\star K(G_1\otimes G_2,
2)$. By an very similar argument to that of Proposition
\ref{prop:pointed-hlevel}, this pointed function type is again a
$1$-type, which justifies set-elimination being applied to
$y$. Combining this with Lemma \ref{lem:Evan}, it is enough to show
that
  \begin{align*}
    x \smile_k y = - c_{2}(y \smile_k x)
  \end{align*}
  for $x : L(G_1)$ and $y : L(G_2)$. We do this by $L(G_1)$
  induction. When either $x$ or $y$ is a point constructor, the
  identity holds by $\refl$. The remaining case amounts to (by
  evaluation of $c_2$) the following identity
  \begin{align*}
    \ap{x \mapsto \ap{x \smile_k (-)}{\LoopG{h}}}{\LoopG{g}} = \mathsf{flip}(\ap{x \mapsto \ap{x \smile_k (-)}{\LoopG{h}}}{\LoopG{g}}^{-1})
  \end{align*}
  which holds by Lemma~\ref{lem:flip-id}.

  We give a rough sketch of the case $n,m \geq 2$. We may apply
  $K(G_1,n)$-elimination again, by the same argument as in the
  previous case. The crucial step this time is verifying
  \begin{align}
    \label{eq:cup-comm}
    \ap{x \mapsto \ap{x \smile_k (-)}{\merid\,h}}{\merid\,g} = \ap{x
      \mapsto \ap{(-1)^{nm} (x \,\smile_k
        (-))}{\merid\,h}}{\merid\,g}
  \end{align}
We note that the above identity and the identities that follow only
are well-typed up to some coherences which we brush under the rug for
the sake of readability. We notice that \eqref{eq:cup-comm} follows if
we can show that for $x : K(G_1,n-1)$, $y : K(G_2,m-1)$, we have
\begin{align}
  \label{eq:cup-comm-alt}
    \ap{x \mapsto \ap{x \smile_k (-)}{\sigma_{m-1}(y)}}{\sigma_{n-1}(x)} = \ap{x
      \mapsto \ap{(-1)^{nm} (x \,\smile_k
        (-))}{\sigma_{m-1}(y)}}{\sigma_{n-1}(x)}
\end{align}
Let us, for further readability, omit the equivalence $c_{p}$
in the following equations. Some of the
following equalities hold up to multiplication by $(-1)^p$ for some $p
: \mathbb{N}$; this will be indicated in the right-hand column.
\begin{align*}
  \ap{a \mapsto \ap{a \smile_k (-)}{\sigma_{m-1}(y)}}{\sigma_{n-1}(x)}
  &= \ap{a \mapsto \ap{(-) \smile_k a}{\sigma_{n-1}(x)}}{\sigma_{m-1}(y)} & (-1)\\
  &= \ap{\sigma_{(n-1)+m}}{\ap{x \smile_k (-)}{\sigma_{m-1}(y)}} \\
  &= \ap{\sigma_{m+(n-1)}}{\ap{(-) \smile_k x}{\sigma_{m-1}(y)}} & m(n-1) \\
  &= \ap{\sigma_{(m-1)+(n-1)+1}}{\sigma_{(m-1)+(n-1)}(y \smile_k x)} \\
  &= \ap{\sigma_{{(n-1)+(m-1)+1}}}{\sigma_{{(n-1)+(m-1)}}(x \smile_k y)} & (n-1)(m-1) \\
  &= \ap{\sigma_{n+(m-1)}}{\ap{(-) \smile_k y}{\sigma_{n-1}(x)}} \\
  &= \ap{\sigma_{m+(n-1)}}{\ap{y \smile_k (-)}{\sigma_{n-1}(x)}} & (m-1)n \\
  &= \ap{a
      \mapsto \ap{(-) \,\smile
        a}{\sigma_{m-1}(y)}}{\sigma_{n-1}(x)}
\end{align*}
\anders{Dubbelkolla kedjan av likheter ovan sen...}

Since $(-1)+n(m-1) + (n-1)(m-1) + (n-1)m =_{\bZ/2\bZ} nm$, the above identity
holds up to multiplication by $(-1)^{nm}$, which gives
\eqref{eq:cup-comm-alt}.
\end{proof}

\subsection{The cup product with ring coefficients}
\label{sec:cupprodringcoeff}

We now consider the special case of $\smile_k \, : K(G_1,n) \times
K(G_2,m) \to K(G_1\otimes G_2,n + m)$ where $G_1 = G_2 = R$ for a (not
necessarily commutative) ring $R$. Let $\mathsf{mult}_{n} : K(R\otimes
R, n) \to K(R,n)$ be the induced map on Eilenberg-MacLane spaces by
the multiplication map $R \otimes R \to R$. Now, consider the
composition
\[\begin{tikzcd}[ampersand replacement=\&]
	{K(R,n)\times K(R,m)} \&\& {K(R\otimes R,n+m)} \&\& {K(R,n+m)}
	\arrow["{\smile_k}", from=1-1, to=1-3]
	\arrow["{\mathsf{mult}_{n+m}}", from=1-3, to=1-5]
\end{tikzcd}\]
Let us, with some overloading of notation, use $\smile_k :
K(R,n)\times K(R,m) \to K(R,n)$ to denote also the composition
above. Note that the above tensor product is a tensor product of
underlying abelian groups and not of rings -- this is of no
consequence for the construction. Using the results of the previous
section, we easily arrive at the following results. Their proofs
follow the same strategy and we will only sketch the proof of
Proposition \ref{prop:cup-comm-ring}.
\begin{proposition}
  \label{prop:cup-props}
  The cup product $\smile_k$ with ring coefficients is associative,
  left- and right-distributive and has $0_k$ as annihilating element.
\end{proposition}
\begin{proposition}
  \label{prop:cup-comm-ring}
  The cup product $\smile_k$ with coefficients in a commutative ring
  is graded-commutative.
\end{proposition}
\begin{proof}
  Let $c_p$ denote the commutator $K(G\otimes H,p) \to K(H \otimes
  G,p)$. Consider the following diagram.
\[\begin{tikzcd}[ampersand replacement=\&]
	{K(R,n)\times K(R,m)} \&\& {K(R\otimes R,n+m)} \&\& {K(R,n+m)} \\
	{K(R,m)\times K(R,n)} \&\& {K(R\otimes R,m+n)} \&\& {K(R,m+n)}
	\arrow["{\smile_k}", from=1-1, to=1-3]
	\arrow[from=1-1, to=2-1]
	\arrow["{\smile_k}", from=2-1, to=2-3]
	\arrow["{\mathsf{mult}_{n+m}}", from=1-3, to=1-5]
	\arrow["{\mathsf{mult}_{m+n}}", from=2-3, to=2-5]
	\arrow["{(-1)^{nm}}", from=1-5, to=2-5]
	\arrow["{c\,\circ\,(-1)^{nm}}"', from=1-3, to=2-3]
\end{tikzcd}\]
The statement is that the outer square commutes. By Proposition
\ref{prop:cup-comm} the left-square commutes. It is easy to verify,
using commutativity of $R$, that $\mathsf{mult}_{n+m} \circ c =
\mathsf{mult}_{m+n}$, making the right-square commute, and we are
done.
\end{proof}
Finally, we note that we now have access to a neutral element,
i.e.\ $1_R : K(R,0)$.
\begin{proposition}
  For $x : K(R,n)$, we have $x \smile_k 1_R = x = 1_R \smile_k x$.
\end{proposition}
\begin{proof}
  By a straightforward induction on $n$, using the recursive
  definition of the cup product.
\end{proof}


==> sections/cohomology.tex <==
\section{Cohomology}
\label{sec:cohomology}

For the construction of cohomology groups, we rely on
\citet{BrownRepr} representability: given $n:\mathbb{N}$, a group $G$
(abelian if $n \geq 1$) and type $X$, we define the \emph{nth
  cohomology group of X with coefficients in $G$} by
%
\begin{align*}
  H^n(X,G) := \truncT{X \to K(G,n)}_0
\end{align*}

These constructions are clearly contravariantly functorial by
pre-composition. The group structure on $K(G,n)$ naturally carries
over to $H^n(X,G)$ by point-wise application of $+_k$ and $-_k$. The
neutral element is, in both cases, the constant map $\_ \, \mapsto
0_k$. In what follows, we will denote addition, inversion and the
neutral element in $H^n(X,G)$ by $+_h$, $-_h$ and $0_h$ respectively.
Explicitly, they are defined by
%
\begin{align*}
  \trunc{f} +_h \trunc{g} &:= \trunc{x \mapsto f(x) +_k g(x)}\\
  -_h \trunc{f} &:= \trunc{x \mapsto -_k f(x)}\\
  0_h &:= \trunc{\_ \, \mapsto 0_k}
\end{align*}

The construction of the cup product with ring coefficients in
Section~\ref{sec:cupprodringcoeff} also extends to our cohomology
groups, giving us a \textit{cup product} on cohomology:
%
\begin{align*}
  \smile \, : H^n(X,R) \times H^m(X,R) \to H^{n+m}(X,R)
\end{align*}
satisfying the usual graded ring axioms and graded commutativity when
$R$ is commutative. In addition, it induces a multiplication on
$H^*(X,R) = \oplus_{n : \mathbb{N}} H^n(X,R)$, turning it into a
graded-commutative ring known as the \emph{cohomology ring} of $X$
with coefficients in $R$. This was formalised in \CubicalAgda
by~\citet{CohomRings23}.
%
This gives an even more fine-grained invariant than just the
cohomology groups $H^n(X,G)$, as it can help to distinguish spaces for
which all cohomology groups agree. As a classical example which was
also considered by \citet{CohomRings23}, consider
Figure~\ref{fig:torusandmickeymouse} which depicts a torus and the
``Mickey Mouse space'' consisting of a sphere glued together with two
circles.

\begin{figure}[h!]
  \centering
  \begin{mathpar}
    \begin{tikzpicture}[scale=0.5]
      \useasboundingbox (-3,-1.5) rectangle (3,1.5);
      \draw[color=blue!90] (0,0) ellipse (3 and 1.5);
      \begin{scope}
        \clip (0,-1.8) ellipse (3 and 2.5);
        \draw[color=blue!90] (0,2.2) ellipse (3 and 2.5);
      \end{scope}
      \begin{scope}
        \clip (0,2.2) ellipse (3 and 2.5);
        \draw[color=blue!90] (0,-2.2) ellipse (3 and 2.5);
      \end{scope}
      \draw[color=blue!90] (0,-1.5) to[bend right=100] (0,-0.3);
      \draw[color=blue!90,densely dotted] (0,-1.5) to[bend left=100] (0,-0.3);
    \end{tikzpicture}
    \and
    \begin{tikzpicture}[scale=0.5]
      \draw[color=blue!90](0.5,0) circle (1.5);

      \draw[color=blue!90](0.5,1.55) circle (0.6);
      \draw[color=blue!90](-2.35,1.55) circle (0.6);
      \draw[color=blue!90] (-2.4,0) to[bend right=40] (0.58,0);
      \draw[color=blue!90,densely dotted] (-2.4,0) to[bend left=40] (0.58,0);
    \end{tikzpicture}
  \end{mathpar}
  \caption{$\mathbb{T}^2$ and $\mathbb{S}^2 \vee \mathbb{S}^1 \vee \mathbb{S}^1$.}
  \label{fig:torusandmickeymouse}
\end{figure}

Let $X$ be either of the two spaces in the figure; one can prove that
$H^0(X,\bZ) \cong \bZ$ as they are connected, $H^1(X,\bZ) \cong \bZ
\times \bZ$ as they each have two 2-dimensional holes (the circle in
the middle of the torus and the one going around the interior, and the
``ears'' of Mickey), and $H^2(X,\bZ) \cong \bZ$ as they have one
3-dimensional hole each (the interior of the torus and Mickey's
head). Furthermore, their higher cohomology groups are all trivial as
they do not have any further higher dimensional cells. The cohomology
groups are hence insufficient to tell the spaces apart. However, one
can show that the cup product on $\mathbb{S}^2 \vee \mathbb{S}^1 \vee
\mathbb{S}^1$ is trivial, while for $\mathbb{T}^2$ it is not. So
$H^*(\mathbb{S}^2 \vee \mathbb{S}^1 \vee \mathbb{S}^1,\bZ) \not \cong
H^*(\mathbb{T}^2,\bZ)$, which again means that the spaces cannot be
continuously deformed into each other.
%
\todo{Släng in en framåtreferens till beräkningsbeviset om vi har
  med det? Bevis i HoTT?}

\subsection{Reduced cohomology}
\label{sec:reduced}

When $X$ is pointed, we may also define \emph{reduced} cohomology
groups by simply requiring all functions to be pointed:
%
\begin{align*}
  \widetilde{H}^n(X,G) := \truncT{X \to_\star K(G,n)}_0
\end{align*}

Just like above the group structure on $K(G,n)$ carries over directly
to $\widetilde{H}(X,G)$. As we will soon see, this definition is
equivalent to the non-reduced version when $n\geq 1$ but has the
advantage of vanishing when $n = 0$.

\begin{proposition}
  The first projection (sending a pointed map to its underlying
  function) induces an isomorphism
  $\widetilde{H}^n(X,G) \cong H^n(X,G)$ for $n \geq 1$.
\end{proposition}
\begin{proof}
  Let $F$ denote the function in question. The fact that it is a
  homomorphism is trivial. We may construct its inverse $F^{-1} :
  H^n(X,G) \to \widetilde{H}^n(X,G)$ explicitly by
  \begin{align*}
    F^{-1}\,\trunc{f}= \trunc{ x \mapsto f(x) -_k f(\star_X)}
  \end{align*}
  In order to see that $F(F^{-1} \trunc{f}) = \trunc{f}$, we note that
  this is a proposition. By the connectedness of $K(G,1)$, we may
  assume we have a path $f(\star_X) = 0_k$. Hence
  \begin{align}\label{eq:red-cohom}
    F(F^{-1}\,\trunc{f})= \trunc{ x \mapsto f(x) -_k f(\star_X)} = \trunc{f}
  \end{align}
  For the other direction, we need to check that
  \begin{align*}
    F^{-1}(F\,\trunc{(f,p)}) = \trunc{(f,p)}
  \end{align*}
  By Lemma \ref{lem:Evan}, we only need to verify that the first
  projections agree, and we are reduced to the second equality
  in~\eqref{eq:red-cohom}, which we have already verified.
\end{proof}

\begin{proposition}
  $\widetilde{H}^0(X,G) \oplus G \cong H^0(X,G)$
\end{proposition}
\begin{proof}
  We define $\phi : (X \to_\star G) \times G \to (X \to G)$ by
  \[
  \phi(f,g) := x \mapsto f(x) +_G g
  \]
  and $\psi : (X \to G) \to (X \to_\star G) \times G$ by
  \[
  \psi(f) := ((x \mapsto f(x) -_G f(\star_X)) , f(\star_X))
  \]
  The fact that these maps cancel out follows immediately from the
  group laws on $G$. This induces an equivalence $H^0(X,G) \simeq
  \widetilde{H}^0(X,G) \oplus G$. The fact that it is an isomorphism
  is also trivial using the group laws on $G$.
\end{proof}

%% \begin{proposition}\label{proposition:H0-contr}
%%   When $X$ is connected, $\widetilde{H}^0(X,G)$ is contractible.
%% \end{proposition}
%% \begin{proof}
%%   \anders{Dubbelkolla detaljerna och korrläs}
%%   It suffices to show that for any $f: X \to_\star G$, the function
%%   $f$ equal (as pointed functions) to the constant function. Since
%%   $G$ is a set, it suffices, by function extensionality, to prove that
%%   $f(x) = 0_G$ for $x : X$. By our connectivity assumption, we have an
%%   element $\truncT{x = \star_X}_{-1}$. Since $G$ is a set, the path
%%   type $f(x) = 0_G$ is a proposition. Hence, we may assume $x =
%%   \star_X$ and it thus suffices to show that $f(\star_X) = 0_k$
%%   which is true on account of $f$ being pointed.
%% \end{proof}

\subsection{Eilenberg-Steenrod axioms for cohomology}
\label{sec:eilenbergsteenrodaxioms}
\axel{Dubbelkolla att alla A/B har blivit X/Y rätt här (det var rörigt innan)}

In order to verify that our cohomology theory is sound, let us verify
the \emph{Eilenberg-Steenrod Axioms}~\cite{eilenberg1952foundations}
for the reduced version of cohomology $\widetilde{H}^n(X,G)$. These
axioms have been studied previously in HoTT by
\citet{ShulmanBlog13,CavalloMsc15,BuchholtzFavonia18,FlorisPhd}. To
state the \textbf{Exactness} axiom, we need to introduce cofibers
(also known as \emph{mapping cones}).

\begin{definition}
  Given a function $f : X \to Y$, the cofibre of $f$, denoted
  $\cofib{f}$, is pushout of the span
  $\mathbbm{1} \leftarrow X \xrightarrow{f} Y$. We will use the name
  $\cfcod$ for the inclusion $\mathsf{inr}: Y \to \cofib{f}$.
\[\begin{tikzcd}[ampersand replacement=\&]
	X \&\& Y \\
	\\
	{\mathbbm{1}} \&\& {\mathsf{cofib\,f}}
	\arrow["f", from=1-1, to=1-3]
	\arrow[from=1-1, to=3-1]
	\arrow[from=3-1, to=3-3]
	\arrow["{\mathsf{cfcod}}", from=1-3, to=3-3]
	\arrow["\lrcorner"{anchor=center, pos=0.125, rotate=180}, draw=none, from=3-3, to=1-1]
\end{tikzcd}\]
\end{definition}

We will also need \emph{wedge sums}.

\begin{definition}
  A family of pointed types $X_i$ and indexing type $i:I$, the wedge
  sum of $X_i$, denoted $\bigvee_i X_i$, is the cofibre of the
  inclusion $j : I \to \Sigma_{i:I}X_i$ defined by
  $j(i) = (i,\star_{X_i})$.
\end{definition}

From a constructive point of view, we will primarily be interested in
wedge sums indexed by a type satisfying the set-level axiom of choice
(see e.g.\ \citep[Section 3.2.3]{CavalloMsc15}, \citep[Section
5.4]{FlorisPhd}, and \citep[Section 6]{BuchholtzFavonia18} for further
discussions of this).

\begin{definition}
  A type $I$ is said to satisfy the set-level axiom of choice
  ($\mathsf{AC}_0$) if for any family of types $X_i$ over $I$, the
  canonical map
  \[
  \truncT{(i : I) \to X_i}_0 \to \left((i : I) \to \truncT{X_i}_0\right)
  \]
  is an equivalence.
\end{definition}
In particular, any finite set $I$ satisfies $\mathsf{AC}_0$. We may
now state the Eilenberg-Steenrod axioms for reduced cohomology. Let us
define $\widetilde{H}^n(X,G) = \mathbbm{1}$ for $n < 0$.
%
\begin{definition}
  A $\bZ$-indexed family of contravariant functors
  $E^n : \mathcal{U}_\star \to \mathsf{AbGroup}$ is said to be an
  ordinary, reduced cohomology theory if the following axioms hold.
  \begin{itemize}
  \item \textbf{Suspension:} there is an isomorphism
    $E^n(X) \cong E^{n+1}(\Sigma\,X)$ natural in $X$.

  \item \textbf{Exactness:} given a function $f : X \to_\star Y$,
    there is an exact sequence
%
  \begin{align*}
    E^n(\cofib{f}) \xrightarrow{E^n \,\cfcod} E^n(Y) \xrightarrow{E^n\,f} E^n(X)
  \end{align*}

  \item \textbf{Dimension:} for $n : \mathbb{Z}$ with $n \neq 0$, we have
  $E^n(\mathbb{S}^0) \cong \mathbbm{1}$.

\item \textbf{Additivity:} for $n : \mathbb{Z}$ and a family of
  pointed types $X_i$ over a type $I$ satsfying $\mathsf{AC}_0$, the
  map $E^n(\bigvee_i X_i) \to \Pi_{i:I}(E^n(X_i))$ induced by the
  functorial acion of $E^n$ on the inclusion
  $X_i \to \bigvee_{i:I} X_i$ is an isomorphism of groups.
  \end{itemize}
\end{definition}

The following theorem was originally proved in Book HoTT by
\citet{CavalloMsc15}. We spell out some of the details for our setup here.

\begin{theorem}
  Given an abelian group $G$, the reduced cohomology theory
  $\widetilde{H}^n(-,G)$ satisfies the Eilenberg-Steenrod Axioms.
\end{theorem}
\begin{proof}
  We verify that   $\widetilde{H}^n(-,G)$ satisfies the four axioms:
  \begin{itemize}
  \item \textbf{Suspension:} this axiom is trivially satisfied when
    $n < -1$. When $n = -1$, we need to verify that
    $\widetilde{H}^0(\Sigma\,X,G)$ is trivial, which follows
    immediately by connectedness of $\Sigma\,X$.
%    \anders{Finns detta i
%     HoTT boken? -- Bara mer generellt i sats 8.2.1 men vårt fall är så trivialt att jag undrar om vi verkligen behöver nån referens... ---- OK, kommenterar. Vi kan fixa om någon klagar}.
    For $n \geq 0$, the suspension axiom follows
    immediately from the fact that $\Sigma$ and $\Omega$ are adjoint.
    %\anders{Var har detta bevisats i Book HoTT?  Hittar inte i HoTT
    %  boken... Evans bevis är ganska långt även om det nog inte så
    %  svårt (iaf inte kubiskt...) -- Vet inte var det först bevisades, men det är så pass trivialt att jag inte tycker referens känns viktigt. Men om du vill köra på Evans bevis, lägg gärna till det --- OK, tar och kommenterar detta. Vi kan fixa om någon klagar}.
    We have
  \begin{align*}
    \widetilde{H}^{n+1}(\Sigma\,X,G) &= \truncT{\Sigma X \to_\star K(G,n+1)}_0 \\
    &\simeq \truncT{X \to_\star \Omega \,K(G,n+1)}_0 \\
    &\simeq \truncT{X \to_\star K(G,n)}_0 \\
    &= \widetilde{H}^n(X,G)
  \end{align*}
  It is easy to see that the above equivalence of types is a
  homomorphism. This concludes the proof of the suspension
  axiom.

\item \textbf{Exactness:} when $n < 0$, there is nothing to prove
  since all groups vanish.
  \axel{Är allt verkligen rätt här? Vi ska väl visa att $\ker(\widetilde{H}^n(f)) = \im{\widetilde{H}^n(\cfcod)}$?}
  Let us consider the case $n \geq 1$. For $\ker(f^*) \subset
  \im{\cfcod^*}$ \axel{Varför asterisker?}, let $\trunc{g} : H^n(Y)$ \axel{Borde det inte vara ett tilde på H?} be an element of
  $\ker(f^*)$ \axel{Varför asterisk?}. We get a homotopy $p : (x : X) \to 0_k =
  g(f(x))$. Using this, we construct a function $g_{\mathsf{cf}} :
  \cofib{f} \to K(G,n)$ by
  \begin{align*}
    g_{\mathsf{cf}}(\inl{\star}) &= 0_k \\
    g_{\mathsf{cf}}(\inr{y}) &= g(y) \\
    \ap{g_{\mathsf{cf}}}{\mathsf{push}\,x} &= p(x)
  \end{align*}
  The fact that $\cfcod^*(\trunc{g_{\mathsf{cf}}}) = \trunc{g}$
  holds by construction. \axel{Kanske var jag förvirrad av detta pga typos?}

  \axel{Om jag inte är ute och cyklar ovan är det typos här med}
  For the other direction, $\im{\cfcod^*} \subset \ker(f^*)$, we want
  to show that the composition $f^* \circ \cfcod^*$ is
  null-homotopic. This holds by construction, since
  $\cfcod \circ f : A \to \cofib{f}$ is null-homotopic by definition
  of $\cofib{f}$.

\item \textbf{Dimension:} when $n < 0$, the statement is trivial. When
  $n > 0$, we have
\begin{align*}
  \widetilde{H}^n(\mathbb{S}^0,G) = \truncT{\mathbb{S}^0 \to_\star K(G,n)}_0 \simeq \truncT{K(G,n)}_0
\end{align*}
Since $K(G,n)$ is $(n-1)$-connected, $\truncT{K(G,n)}_0$
\axel{Är trunkeringen viktig här?}
vanishes for $n > 0$.
\axel{Kanske säga ``$K(G,n)$ vanishes for $n > 0$ and hence does $\truncT{K(G,n)}_0$ as well.'' istället?}

\item \textbf{Additivity:} again, the statement is trivial when
  $n < 0$. For the non-trivial case, the lemma follows from a simple
  rewriting of $H^n(\bigvee_{i:I} X_i,G)$ using the elimination
  principle for $\bigvee_{i:I}$:
\begin{align*}
  \widetilde{H}^n\left(\bigvee_{i:I} X_i,G\right) &:= \bigg\Vert \bigvee_{i:I} X_i \to_\star K(G,n) \bigg\Vert_0 \\
  &\simeq \Bigg\Vert \sum_{f : (\sum_{i:I} X_i) \to K(G,n)} \sum_{x_0 : K(G,n)} \left(((i : I) \to f(i,\star_{A_i}) = x_0) \times (x_0 = 0_k)\right) \Bigg\Vert_0\\
  &\simeq \Bigg\Vert\sum_{f : (\sum_{i:I} X_i) \to K(G,n)} ((i : I) \to f(i,\star_{A_i}) = 0_k) \Bigg\Vert_0 \times \Bigg\Vert \sum_{x_0 : K(G,n)} (x_0 = 0_k)  \Bigg\Vert_0 \\
  &\simeq \Bigg\Vert\sum_{f : (\sum_{i:I} X_i) \to K(G,n)} ((i : I) \to f(i,\star_{A_i}) = 0_k) \Bigg\Vert_0 \\
  &\simeq \truncT{(i : I) \to X_i \to_\star K(G,n)}_0\\
  &\simeq (i : I) \to \truncT{X_i \to_\star K(G,n)}_0 & (\mathsf{AC}_0)\\
  &= \Pi_{i:I}\widetilde{H}^n(X_i,G)
\end{align*}
where the step from the second to the third line i
The fact that this composition of equivalences indeed gives the usual homomorphism $\widetilde{H}^n\left(\bigvee_{i:I} X_i,G\right) \to \Pi_{i:I}\widetilde{H}^n(X_i,G)$ is immediate by construction.
\anders{Jag fattar inte sista kommentaren. Och måste vi inte säga något om varför detta är en gruppisomorfi? -- tydligare nu? Axiomet rör sig om en särskild homomorfi som alltid går att definiera. Påståendet i axiomet är att just den homomorfin är en ekvivalens}
\axel{Ja, men något verkar ha försvunnit? Iaf börjar det med en ofärdig mening...}
\end{itemize}
\end{proof}

% \anders{Säg nåt om \textit{generalized (Eilenberg-Steenrod)
%     cohomology} på nlab för ej reducerad kohomologi}

% \anders{Säg nåt om att vi kan bevisa saker direkt från axiomen med
%   referens till FB. Övergång till Mayer-Vietoris}

Just like in traditional algebraic topology many standard results and
constructions follow directly from the axioms, see e.g.\
\citep{CavalloMsc15,BuchholtzFavonia18} for concrete examples,
including the Mayer-Vietoris sequence \citep[Section~4.5]{CavalloMsc15}.


% To motivate the usefulness of these axioms, consider the following
% simple cohomology computations. Let $E$ denote an arbitrary cohomology theory.
% \begin{proposition}
%   The cohomology groups $E^n(\mathbbm{1})$ vanish.
% \end{proposition}
% \begin{proof}
%   The map $\mathbbm{1} \to \mathbbm{1} \vee \mathbbm{1}$ defined via
%   inclusion in the left component is an equivalence. This implies, via
%   \textbf{additivity}, that the first projection $E^n(\mathbbm{1})
%   \times E^{n}(\mathbbm{1}) \to E^n(\mathbbm{1})$ is an isomorphism and
%   hence $E^n(\mathbbm{1})$ must be trivial.
% \end{proof}

% \begin{proposition}
%   For any cohomology theory $E$, we have
%   \begin{align*}
%     E^n(\mathbb{S}^{m}) \cong \begin{cases}
%       E^0(\mathbb{S}^{0}) & \text{if $n = m$}\\
%       \mathbbm{1} & \text{otherwise}
%       \end{cases}
%   \end{align*}
% \end{proposition}
% \begin{proof}
%   By iterated application of \textbf{suspension}, we have
%   $E^n(\mathbb{S}^{m}) \cong E^{n-m}(\mathbb{S}^0)$ which, by
%   \textbf{dimension}, we know vanishes when $n - m \neq 0$.
% \end{proof}

% This allows us to compute the cohomology of the cofibre of any map
% $f : \mathbb{S}^n \to \mathbb{S}^m$ (examples of which include
% e.g.\ the complex projective spaces $\mathbb{C}P^{n}$)
% \begin{proposition}
%   For any $f : \mathbb{S}^n \to \mathbb{S}^m$, we have
%   \begin{align*}
%     E^n(\mathsf{cofib}\,f) \cong \begin{cases}
%       s \\
%       s
%       \end{cases}
%   \end{align*}
% \end{proposition}

\subsection{Mayer-Vietoris}
\label{sec:mayervietoris}

The Mayer-Vietoris sequence is surprisingly easy to construct in
HoTT. It was first developed in HoTT by \citet{CavalloMsc15} for
axiomatic cohomology theories and then for the specific
$\bZ$-cohomology theory of \cite{Brunerie16} who constructed the
sequence directly. This direct construction in no way depends on the
use of $\bZ$-coefficients and the exact same proof translates to our
theory. In this short section, we will briefly recall this
construction. All notations are borrowed from \citet{Brunerie16}.

Consider three types $X,Y,Z$ with functions $f : X \to Y$ and
$g : X \to Z$. Let $D$ denote the pushout of the span
$Y \xleftarrow{f} X \xrightarrow{g} Z$. There is a natural map
$\widetilde{d} : (X \to K(G,n)) \to (D \to K(G,n+1))$ given by
\begin{align*}
  \widetilde{d}(\gamma)(\inl{y}) &:= 0_k \\
  \widetilde{d}(\gamma)(\inr{z}) &:= 0_k \\
  \ap{\widetilde{d}(\gamma)}{\push{x}} &:= \sigma_n(\gamma(x))
\end{align*}
This lifts to a map $d : H^n(X,G) \to H^{n+1}(X,G)$ by
$d(\trunc{\gamma}) = \trunc{\widetilde{d}(\gamma)}$. There is also a
natural map $\Delta : H^{n}(Y) \times H^{n}(Z) \to H^n(X,G)$ given by
\[
  \Delta(\alpha,\beta) := f^*(\alpha) -_h g^*(\beta)
\]
Finally, we have a map $i : H^n(D,G) \to H^n(Y,G) \times H^n(Z,G)$ given by
\[
  i(\delta) := (\inl{}^*(\delta), \inr{}^*(\delta))
\]

\begin{theorem}[Mayer-Vietoris sequence]
  The families of functions $i$, $\Delta$ and $d$ give rise to a long
  exact sequence on the form:
\[\begin{tikzcd}[ampersand replacement=\&]
	{H^0(D,G)} \&\& {H^0(Y,G) \times H^0(Z,G)} \&\& {H^0(X,G)} \\
	{H^1(D,G)} \&\& {H^1(Y,G) \times H^1(Z,G)} \&\& {H^1(X,G)} \\
	{H^2(D,G)} \&\& \dots
	\arrow["i", from=1-1, to=1-3]
	\arrow["\Delta", from=1-3, to=1-5]
	\arrow["d"', from=1-5, to=2-1,bend right=2]
	\arrow["i",,from=2-1, to=2-3]
	\arrow["\Delta", from=2-3, to=2-5]
	\arrow["d"', from=2-5, to=3-1,bend right=2]
	\arrow["i",,from=3-1, to=3-3]
\end{tikzcd}\]
\end{theorem}
\begin{proof}
  Straightforward generalisation of
  \citet[Proposition~5.2.2]{Brunerie16}.
\end{proof}

This is useful to compute cohomology of spaces defined as pushouts,
e.g.\ $\mathbb{C}P^2$ (see Section \ref{sec:cp2}). Another useful long exact
sequence developed in HoTT by \citet{Brunerie16} is the Gysin sequence.

%% We first show that any composition in the diagram is trivial.
%% For the composition $\Delta \circ i : H^n(D,G) \to H^n(X,G)$ this is direct since
%% \[\Delta(i(\trunc{\delta})) = f^*(\inl{}^*(\delta)) -_h g^*(\inr{}^*(\delta)) \]
%% and $f^*(\inl{}^*(\delta)) = g^*(\inr{}^*(\delta))$ by definition of $D$.

%% For the composition $d \circ \Delta$, we have
%% \begin{align*}
%%   (d \circ \Delta)(\trunc{\alpha},\trunc{\beta}) = \trunc{\widetilde{d}(\alpha \circ f)} -_h \trunc{\widetilde{d}(\beta \circ g)}
%% \end{align*}
%% by construction.
%% We are done if we can show that $\delta(\widetilde{d}(\alpha \circ f))(x) = \delta(\widetilde{d}(\beta \circ g))(x)$ for $d : D$. We do this by induction on $d$. Since both sides compute to $0_k$ when $x$ is a point constructor and, respectively, to $\sigma(\alpha(f(-)))$ and $\sigma(\beta(g(-)))$ for path constructors, the problem amount to providing the following data:
%% \begin{itemize}
%%   \item A family of paths $p : Y \to 0_k = 0_k$
%%   \item A family of paths $q : Z \to 0_k = 0_k$
%%   \item For every $x:X$, a filler of the square
%% \[\begin{tikzcd}[ampersand replacement=\&]
%% 	{0_k} \&\& {0_k} \\
%% 	\\
%% 	{0_k} \&\& {0_k}
%% 	\arrow["{\sigma(\beta(g(x)))}", from=1-1, to=1-3]
%% 	\arrow["{\sigma(\alpha(f(x)))}"', from=3-1, to=3-3]
%% 	\arrow["{q(g(x))}"', from=3-3, to=1-3]
%% 	\arrow["{p(f(x))}", from=3-1, to=1-1]
%% \end{tikzcd}\]
%% \end{itemize}
%% We define $p(y) : \sigma(\alpha(y))$ and $q(z) = \sigma(\beta(z))$, and the square filling problem reduces to proving that $\sigma(\alpha(f(x)))^{-1} \cdot \sigma(\alpha(f(x))) \cdot \sigma(\beta(g(x))) = \sigma(\beta(g(x)))$, which of course is trivial. \todo{Doublecheck this}

%% The final composition to consider is $i \circ d$, which is trivially null by definition of $i$ and $d$.

%% We now show the inclusion $\ker \subset \mathsf{im}$ for the various functions. Let us begin with $\ker(i)\subset\im{d}$. Let $\trunc{\delta} : H^{n+1}(D,G)$ and suppose that $i(\trunc{\delta}) = (0_h,0_h)$. This (merely) gives us homotopies $p : (y : Y) \to \delta (\inl{y}) = 0_k$ and $q : (z : Z) \to \delta(\inr{z})$. For $x : X$, we get a loop $l(x) : \Omega(K(G,n+1))$ by
%% \[l(x) = p(f(x))^{-1} \cdot \ap{\delta}{\push{x}} \cdot q(g(x))\]
%% The composition $\sigma^{-1} \circ l$ then gives a map $A \to K(G,n)$. We claim that $\delta = \widetilde{d}(\sigma^{-1} \circ l)$. Such a proof is given by providing the following data
%% \begin{itemize}
%% \item A family of paths $r : (y : Y) \to \delta(\inl{y}) = 0_k$
%% \item A family of paths $s : (z : Z) \to \delta(\inr{z}) = 0_k$
%% \item A filler of the square
%%   \[\begin{tikzcd}[ampersand replacement=\&]
%% 	{0_k} \&\& {0_k} \\
%% 	\\
%% 	{\delta(f(x))} \&\& {\delta(g(x))}
%% 	\arrow["{\sigma(\sigma^{-1}(l(x))}", from=1-1, to=1-3]
%% 	\arrow["{\mathsf{ap}_{\delta}(\mathsf{push}\,x)}"', from=3-1, to=3-3]
%% 	\arrow["{s(g(x))}"', from=3-3, to=1-3]
%% 	\arrow["{r(f(x))}", from=3-1, to=1-1]
%%   \end{tikzcd}\]
%% \end{itemize}
%% Using $p \circ f$ for $r$ and $q \circ g$ for $s$, the problem boils down to filling the square
%% \[\begin{tikzcd}[ampersand replacement=\&]
%% 	{0_k} \&\&\& {0_k} \\
%% 	\\
%% 	{\delta(f(x))} \&\&\& {\delta(g(x))}
%% 	\arrow["{p(f(x))}", from=3-1, to=1-1]
%% 	\arrow["{p(f(x))^{-1} \cdot \mathsf{ap}_{\delta}(\mathsf{push}\,x) \cdot q(g(x))}", from=1-1, to=1-4]
%% 	\arrow["{q(g(x))}"', from=3-4, to=1-4]
%% 	\arrow["{\mathsf{ap}_{\delta}(\mathsf{push}\,x)}"', from=3-1, to=3-4]
%% \end{tikzcd}\]
%% which is trivial by definition of path composition, and we are done

%% We now verify that $\ker(\Delta)\subset \im{i}$. Let $(\trunc{\alpha},\trunc{\beta}) : H^n(Y,G) \times H^n(Z,G)$ and suppose that $\Delta (\trunc{\alpha},\trunc{\beta})  = 0_h$. By definition of $\Delta$, this (merely) gives us a homotopy $p : (x : A) \to \alpha (f(x)) = \beta (g(x))$. Let us construct $\delta : D \to K(G,n)$ by
%% \begin{align*}
%%   \delta(\inl{y}) &= \alpha(y) \\
%%   \delta(\inr{z}) &= \beta(z) \\
%%   \ap{\delta}{\push{x}} &= p(x)
%% \end{align*}
%% By definition, we have $i(\trunc{\delta}) = (\trunc{\alpha},\trunc{\beta})$.

%% Finally, let us verify $\ker(d) \subset \im{\Delta}$. Let $\trunc{\gamma} : H^n(X,G)$ and suppose theat $d(\gamma) = 0_h$. This (merely) gives us a homotopy $(w : D) \to \widetilde{d}(\gamma) = 0_h$, which in turn can be broken down to the following data:
%% \begin{itemize}
%% \item A family of loops $p : Y \to \Omega K(G,n+1)$
%% \item A family of loops $q : Z \to \Omega K(G,n+1)$
%% \item A homotopy $r : (x : X) \to p(f(x))^{-1} \cdot \sigma(\gamma(x)) \cdot q(g(x)) = \refl$
%% \end{itemize}
%% Applying $\sigma^{-1}$ and shuffling the homotopy, the above data is tranformed to
%% \begin{itemize}
%% \item A function $\alpha : Y \to K(G,n)$
%% \item A function $\beta : Z \to K(G,n)$
%% \item A homotopy $(x : X) \to \gamma(x) = \alpha(f(x)) -_k \beta(g(x))$
%% \end{itemize}
%% Hence, $\Delta(\trunc{\alpha},\trunc{\beta}) = \trunc{\gamma}$, and we are done.

\subsection{The Thom isomorphism and the Gysin sequence}
\label{sec:gysin}

\citet{Brunerie16} also introduced, for the first time in HoTT, the
Thom isomorphism and the Gysin sequence. While Brunerie's original
constructions concerned integral cohomology, we may easily generalise
them to cohomology with coefficients in an arbitrary commutative ring
$R$. In this short section, we will give a quick review of Brunerie's
proof/construction -- here generalised to arbitrary coefficients
(which has no major effect on the proofs).

Let $\alpha_n : \mathbb{S}^n \to_\star K(R,n)$ denote the image of
$1_r : R$ under the equivalence
\begin{align*}
  R \simeq \Omega^n K(R,n) \simeq (\mathbb{S}^n \to_\star K(R,n))
\end{align*}
This induces a family of equivalences
$g^i : K(R,i) \to (\mathbb{S}^n \to_\star K(R,i + n))$ defined by
\begin{align*}
  g^i(x) := y\mapsto x \smile_k \alpha_n(y)
\end{align*}
Now, let $B$ be a $0$-connected, pointed type and suppose we have
fibration $Q : B \to \mathsf{Type}_\star$ with
$\psi : Q(\star_B) \simeq_\star \mathbb{S}^n$ and a $B$-indexed family
of functions $c_b : Q(b) \to_\star K(R,n)$ with
$c_{\star_B} = \alpha_n \circ \psi$. We remark that such a family
automatically exists when $B$ is further assumed to be
$1$-connected. We may use this to define a $B$-relative version of
$g^i$:
\begin{align*}
  g_b^i &: K(R,i) \to (Q(b) \to_\star K(R,i+n))\\
  g_b^i(x) &:= y \mapsto x \smile_k c_b(y)
\end{align*}
Showing that this map is an equivalence is straightforward: for
connectedness reasons, we only need to do so when $b$ is $\star_B$, in
which case we have $g_{\star_B}^i(x) = g^i(x) \circ \psi$ which we
already know defines an equivalence.

The fact that $g_b^i$ is an equivalence means, in particular, that
the following map is one too.
\begin{align*}
  \varphi^i &: (B \to K(R,i)) \to ((b : B) \to Q(b) \to_\star K(R,i+n))\\
  \varphi^i(f) &:= (b,q \mapsto f(b) \smile c_b(q))
\end{align*}
We instantiate the above with some concrete spaces. Let
$P : B \to \mathsf{Type}_\star$ be a fibration with
$P(\star_B) \simeq_\star \mathbb{S}^{n-1}$ and let
$Q(b)$ be the suspension of $P(b)$, i.e.\ $Q(b) := \Sigma\,(P(b))$.
Suppose also that we have a family
$c_b : (Q(b) \to_\star K(R,n))$ as above (again, this is automatic if
$B$ is $1$-connected). Consider, $E := \Sigma_{b:B}P(b)$, the total
space of $P$ and $\widetilde{E}$ the cofibre of the projection map
$E \to B$. It is easy to see that
$((b : B) \to Q(b) \to_\star K(R,k)) \simeq (\widetilde{E} \to_\star
K(R,k))$. Combining this with $\varphi^i$, we thus get an isomorphism
\begin{align*}
  \phi^i : H^i(B,R) \cong \widetilde{H}^{i+ n}(\widetilde{E},R)
\end{align*}
Finally, we may consider the long exact sequence related to the
pushout defining $\widetilde{E}$ (the first row in the following
diagram). Substituting along $\phi^{i-n}$ yields the Gysin sequence
(the second row in the diagram).
\[\begin{tikzcd}[ampersand replacement=\&]
	\dots \& {H^{i-1}(E,R)} \& {\widetilde{H}^i(\widetilde{E},R)} \& {H^i(B,R)} \& {H^i(E,R)} \& \dots \\
	\dots \& {H^{i-1}(E,R)} \& {H^{i-n}(B,R)} \& {H^i(B,R)} \& {H^i(E,R)} \& \dots
	\arrow["\phi^{i-n}", from=2-3, to=1-3]
	\arrow[from=1-2, to=1-3]
	\arrow[dashed, from=2-2, to=2-3]
	\arrow[Rightarrow, no head, from=2-2, to=1-2]
	\arrow[from=1-1, to=1-2]
	\arrow[from=2-1, to=2-2]
	\arrow["{(-)\smile e}"', from=2-3, to=2-4]
	\arrow[from=1-3, to=1-4]
	\arrow[Rightarrow, no head, from=1-4, to=2-4]
	\arrow[from=1-4, to=1-5]
	\arrow[from=2-4, to=2-5]
	\arrow[from=1-5, to=1-6]
	\arrow[from=2-5, to=2-6]
	\arrow[Rightarrow, no head, from=1-5, to=2-5]
      \end{tikzcd}\]
    Here the dashed arrow is defined as the composition $H^{i-1}(E,R) \to \widetilde{H}^i(\widetilde{E},R) \xrightarrow{(\phi^{i-n})^{-1}} H^{i-n}(B,R)$.

Above, the class $e : H^n(B,R)$ is defined by
$e := \trunc{b \mapsto c_b(\mathsf{south})}$. The commutativity of the
centre square follows immediately by construction of $\phi^{i-n}$. For
the sake of completeness, let us state the existence of the Gysin
sequence as a theorem.
\begin{theorem}[The Gysin Sequence]\label{thm:Gysin}
  Let $B$ be $0$-connected and $P : B \to \mathsf{Type}$ be a
  fibration equipped with a pointed equivalence
  $\psi : P(\star_B) \simeq \mathbb{S}^{n-1}$. Assume that the
  following condition is satisfied
  \begin{enumerate}[($\ast$)]
  \item There is a $B$-indexed family
    $c_b : \Sigma(P(b)) \to_\star K(R,{n})$ s.t.\ $c_{\star_{B}}$ is
    the image of $1_R : R$ under the composition of isomorphisms
    \[
      R \cong H^n(\mathbb{S}^n,R)\, \overset{\Sigma(\psi)}{\cong}\,
      H^n(\Sigma(P(\star_B)),R)
      \]\label{gysin-cond}
  \end{enumerate}
  Let $E$ denote the total space of $P$ and define $e : H^n(B,R)$ by $e :=
\trunc{b \mapsto c_b(\mathsf{south})}$. We get a long exact sequence
\[\begin{tikzcd}[ampersand replacement=\&]
	\dots \& {H^{i-1}(E,R)} \& {H^{i-n}(B,R)} \& {H^i(B,R)} \& {H^i(E,R)} \& \dots
	\arrow[from=1-2, to=1-3]
	\arrow["{(-)\smile e}", from=1-3, to=1-4]
        \arrow[from=1-1,to=1-2]
	\arrow[from=1-4, to=1-5]
	\arrow[from=1-5, to=1-6]
\end{tikzcd}\]
Moreover, condition \hyperlink{gysin-cond}{($\ast$)} is always satisfied when $B$ is $1$-connected.
\end{theorem}

The Gysin sequence was for instance crucially used
in~\cite{Brunerie16} to compute the integral cohomology \emph{ring} of
$\mathbb{C}P^2$ (see also Section \ref{sec:cp2}). We will also use this sequence to compute the cohomology ring of the infinite projective space in Section \ref{sec:rpinf}.


==> sections/computations.tex <==
\section{Something about computations}
\label{sec:computations}

\todo{Det här stycket kan vi renskriva och fixa klart när allt annat
  är klart. Jag vill ha benchmarks och öppna problem i stil med mitt
  talk på HoTT konferensen 2023}

\todo{Vi kan citera vår LICS artikel och diskutera varför det
  fortfarande är intressant med nya beräkningar (den ursprungliga
  definitionen är inte beräknad t.ex.)}

\todo{Påminn om att detta är enda delen som kräver att univalence och
  HITs går att beräkna med. Prata kanske lite om formaliseringen i
  Cubical Agda också?}

\todo{Dela upp i delstycken?}

A great advantage of computer formalisation of mathematics is that it
opens up for the possibility of `proofs by computation'. Suppose, for
instance, that you want to show that $g : G$, an element of interest
in some concrete group, is non-trivial. A typical approach to this
problem is to consider a homomorphism to some other well-known group,
say a homomorphism $\phi : G \to \bZ$, and prove that $\phi(g) \neq
0$. The only difficult part of such a proof is of course computing the
value of $\phi(g)$. In a constructive proof assistant like
\CubicalAgda, this is, in theory, never an issue. As soon as we define
a function $G \to \bZ$, we have implicitly designed an algorithm for
converting elements of the first group into elements of the latter. I
particular, we may simply ask \CubicalAgda to \emph{normalise}
$\phi(g)$; if we give \CubicalAgda enough time and memory, we can
always expect it to return an output.

There have been some successes to this end already \todo{cite other
  stuff stuff using computation}. One typical textbook exercise in the
applications of cohomology rings is to show that the wedge sum of a
circle and a sphere is not homotopy equivalent to the torus by
distinguishing their cohomology rings. The problem boils down to
showing that the cup product vanishes in degrees $(1,1)$ for
$\mathbb{S}^1\vee \mathbb{S}^2$ but not for $T^2$. This was done
computationally by \citet{BLM} by running the following function in
\CubicalAgda
\[
\mathbbm{1}\xrightarrow{(1,0),(0,1)}(\bZ \times \bZ) \times (\bZ \times \bZ) \xrightarrow{\cong} H^1(X,\bZ) \times H^1(X,\bZ) \xrightarrow{\smile} H^2(X,\bZ) \xrightarrow{\cong} \bZ
\]
for $X \in \{\mathbb{S}^1\vee \mathbb{S}^2,T^2\}$. Simply by noting
that the output was $0$ for one space and $1$ for the second, one can
deduce that $\mathbb{S}^1\vee \mathbb{S}^2 \not\simeq T^2$.

Unfortunately, the feasibility of these methods is rather limit in
currently existing proof assistants. Perhaps the most well-known
example from HoTT is that of the Brunerie number: that is, the number
$n : \bZ$ such that $\pi_4(\mathbb{S}^3) \cong \bZ/n\bZ$. The number
$n$ can, in theory, be computed by running the function
\[
\mathbbm{1}\xrightarrow{(1,1)}\bZ \times \bZ \xrightarrow{\cong}
\pi_2(\mathbb{S}^2) \times \pi_2(\mathbb{S}^2) \xrightarrow{[-,-]}
\pi_3(\mathbb{S}^2) \xrightarrow{\cong} \bZ
\]
where $[-,-]$ denotes the Whitehead product~\todo{ref}. Brunerie
dedicates the second half of his PhD thesis to proving manually that
the absolute value of the number returned by this function is $2$. To
this end, he has to introduce cohomology, the Hopf invariant and
several other constructions. If this computation were to be
successful, however, these manual computations would not be required in
Brunerie's proof of $\pi_4(\mathbb{S}^3) \cong \bZTwo$. Unfortunately,
we still have not been able to successfully carry out this computation
in \CubicalAgda or any other constructive proof
assistant. \todo{anders: some techincal reason why you think this is?}

In order to understand what is going wrong with the Brunerie number,
it is useful to do some benchmarking. To do this, we would like to
introduce some other constructively defined numbers of (at least some)
mathemtical importance which we, in theory, should be able to compute
in \CubicalAgda. Already in Brunerie's thesis, another such number
appears; namely, the output of the following function
\begin{align}\label{mini-brunerie}
\mathbbm{1}\xrightarrow{(1,1)}\bZ \times \bZ \xrightarrow{\cong}
H^2(\CP,\bZ) \times H^2(\CP,\bZ) \xrightarrow{\smile} H^4(\CP,\bZ)
\xrightarrow{\cong} \bZ
\end{align}
%
Successfully running it should give an output of absolute value $1$
and would provide a proof that the Hopf invariant $\pi_3(\mathbb{S}^2)
\to \bZ$ is an isomorphism. This computation was attempted
by \citet{BLM} using their definition of $\bZ$-cohomology (of which our
definition is a generalisation) and failed. The definitiion of this
number is arguably less complex than that of the Brunerie number, so
the fact that we fail already here is an indication that a careful
benchmarking of similar examples should be done. We have, in fact,
already in this paper implicitly defined new Brunerie
numbers. Consider, for instance the function
\[
\mathbbm{1} \xrightarrow{\trunc{\alpha},\trunc{\alpha}} H^1(\RP,\bZTwo) \times H^1(\RP,\bZTwo) \xrightarrow{\smile} H^2(\RP,\bZTwo) \xrightarrow{\cong} \bZTwo
\]
where $\alpha : \RP \to K(\bZTwo,1)$ is defined as in Proposition
\ref{prop:RP-cup}. Computing this, we should get output $1$. This
would completely remove the need for Lemma \ref{lem:killDiag-comm} in
the proof. Similar computations could also be used to verify
Proposition \ref{prop:H*-K2-rels}. We judge these computations to be
more feasible than that of~\eqref{mini-brunerie} since the degrees of
the cohomology groups involved are lower.

To get a better idea of which computations succeed and which fail, we
have run several computations on the form $H^n(X,G) \to H$ for
concrete groups $G$ and $H$ and concrete spaces/types $X$. These are
given in Table \ref{benchmarks}. The first column gives the cohomology
group $H^n(X,G)$ we are starting in, the second column describes what
the coefficients $G$ are taken to be and the third column gives the
group $H$ such that there is an isomorphism $\phi : H^n(X,G) \cong
H$. The fourth consists of elements $h : H^n(X,G)$ for which we have
attempted to run $\phi(h)$ in \CubicalAgda. Finally, the fifth column
describes the time it takes for \CubicalAgda to run the
computation. Computations which fail to terminate within $10$ minutes
will be marked by \xmark. If a certain cohomology group $H^n(X,G)$ is
isomorphic to a cyclic group, we will simply write $\mathsf{gen}$ for
its generator.

\begin{center}
\begin{table}
  \label{benchmarks}
\begin{tabular}{ |c|c|c|c|c| }
 \hline
 Cohomology group & Coefficients & Isomorphic to & Element & Runtime \\
 \hline
 $H^1(\mathbb{S}^1,-)$
 & \begin{tabular}{@{}cc@{}}
     $\bZ$ \\
     $\bZTwo$
   \end{tabular}
 &  \begin{tabular}{@{}cc@{}}
     $\bZ$ \\
     $\bZTwo$
   \end{tabular}
 & \begin{tabular}{@{}cc@{}}
     \textsf{gen} \\
     \textsf{gen}
     \end{tabular}
 & \begin{tabular}{@{}cc@{}}
     10ms \\
     3ms
     \end{tabular} \\
 \hline
 \todo{Finish this} & cell8 & cell9 & asd & 100000000 s\\ 
 \hline
\end{tabular}
  \caption{Benchmarks}
\end{table}
\end{center}


==> sections/conclusions.tex <==
\section{Conclusion etc}

\anders{Diskutera future work och vad vi lärt oss av den här
  formaliseringen?}


==> sections/direct.tex <==
\section{Computations of cohomology groups and rings}
\label{sec:direct}

In this section we will compute some cohomology groups and rings of
some classical spaces. All of these groups/rings will be very familiar
to the traditional mathematician. Our intent is to showcase how these
computations are carried out in HoTT. What is particularly interesting
here is that the computations can often be done very directly, without
relying on more general machinery (e.g.\ the Mayer-Vietoris sequence,
spectral sequences, etc.). We have two reasons for doing so. Firstly,
we think that this in many cases showcases the strength of working
with cohomology synethetically in HoTT. Many proofs become incredibly
short and rely solely on spelling out the computation rule for the
space in question. In particular, we can carry these proofs out
without any homological algebra. Secondly, by carefully choosing the
direct proofs, we often produce proof terms which are far simpler than
those produced by more advanced machinery. This means that we can use
the isomorphisms we construct here to make concrete computations
(i.e.\ normalisations of closed terms) in a constructive proof
assistant such as \CubicalAgda. We will discuss this more in
Section~\ref{sec:computations}.

\todo{Lägg in en tabell över allt som kommer här?}

\todo{Lägg även till en kort kommentar om tidigare artiklar och vad
  som är nytt här}

Let us start by computing some cohomology groups of some special
types.
\begin{proposition}
  \label{prop:Hn-Unit}
  $H^n(\mathbbm{1}) \cong \begin{cases} G & n = 0 \\ \mathbbm{1} & n \geq 1 \end{cases}$
\end{proposition}
\begin{proof}
  We have $H^n(\mathbbm{1}) := \truncT{\mathbbm{1} \to K(G,n)}_0 \simeq \truncT{K(G,n)}_0$.
This is $\truncT{G}_0 \simeq G$ when $n = 0$ and contractible when $n
> 0$ since $K(G,n)$ is $(n-1)$-connected.
\end{proof}

We also note the following easy lemma
\begin{lemma}
  \label{lem:Hn-Trunc}
  For any space $X$, we have $H^n(X,G) \cong H^n(\truncT{X}_n,G)$
\end{lemma}
\begin{proof}
  Using that $K(G,n)$ is $n$-truncated, we get, by the universal
  property of $n$-truncation, that
  \begin{align*}
    H^n(X,G) = \truncT{X \to K(G,n)}_0 \simeq \truncT{\truncT{X}_n \to K(G,n)}_0 = H^n(\truncT{X}_n,G)
  \end{align*}
  The fact that this equivalence is a homomorphism is trivial.
\end{proof}

Using this, we can easily compute the zeroth cohomology group of a
$0$-connected space (and hence, any $n$-connected space with
$n \geq 0$).
%
\begin{proposition}
  For any $0$-connected space $X$, we have $H^0(X,G) \cong G$.
\end{proposition}
%
\begin{proof}
  By Lemma \ref{lem:Hn-Trunc}, we have $H^0(X,G) =
  H^0(\truncT{X}_0,G)$. But $\truncT{X}_0 \simeq \mathbbm{1}$ since
  $X$ is $0$-connected. Thus, by Proposition \ref{prop:Hn-Unit}, the zeroth
  cohomology group is isomorphic to $G$.
\end{proof}

We now turn our attention to the cohomology groups and rings of some
more interesting spaces.

\subsection{Spheres}

We now have what we need to compute the cohomology of the
$n$-sphere. Let us start with $n = 1$.

\begin{proposition}
    \label{prop:H1-S1}
    $H^1(\mathbb{S}^1,G) \cong G$
  \end{proposition}
  \begin{proof}
    A function $\mathbb{S}^1 \to K(G,1)$ is uniquely determined by its
    action on $\cbase$ and $\Loop$. Hence, it corresponds to choices
    of a point $x : K(G,1)$ and a loop $x = x$. In other words,
    $(\mathbb{S}^1 \to K(G,1)) \simeq \Sigma_{x : K(G,1)} (x =
    x)$. But $K(G,1)$ is homogeneous, so
    $(x = x) \simeq \Omega K(G,1)$. Thus, we have
    %
    \begin{align*}
      H^1(\mathbb{S}^1,G) &= \truncT{\mathbb{S}^1 \to K(G,1)}_0 \\
      &\simeq \truncT{\Sigma_{x : K(G,1)} (x = x)}_0\\
      &\simeq \truncT{K(G,1) \times \Omega K(G,1)}_0 \\
      &\simeq \truncT{K(G,1)}_0 \times G
    \end{align*}
    %
    But $K(G,1)$ is $0$-connected, so $\truncT{K(G,1)}_0$
    vanishes. Thus, we have $H^1(\mathbb{S}^1,G) \simeq G$.

    We need to verify that this isomorphism is a homomorphism. It is
    easier to show that its inverse is. Let us call it $\phi$. By
    definition, $\phi(g) = \trunc{f_g}$ where
    $f_g : \mathbb{S}^1 \to K(G,1)$ is the map sending $\cbase$ to
    $\star$ and $\Loop$ to $\LoopG{g}$. Thus, we only need to verify
    that for $g_1,g_2 : G$ and $x : \mathbb{S}^1$, we have
    $f_{g_1}(x) +_k f_{g_2}(x) = f_{g_1 + g_2}(x)$. We do this by
    induction on $x$. When $x$ is $\cbase$, the goal holds by
    $\refl$. For the action on $\Loop$, we need to show that
    \begin{align*}
      \app{+_k}{\LoopG{g_1}}{\LoopG{g_2}} = \LoopG{(g_1 + g_2)}
    \end{align*}
    which holds by Proposition \ref{prop:ap-+} and functoriality of $\LoopG{}$.
  \end{proof}
  It is easy to generalise this to get all non-trivial cohomology
  groups of $\mathbb{S}^n$.
  \begin{proposition}
    For $n \geq 0$, we have $H^n(\mathbb{S}^n,G) \cong G$.
  \end{proposition}
  \begin{proof}
    The case $n = 0$ is similar to the proof of Proposition
    \ref{prop:H1-S1}. For $n > 1$, we simply apply the suspension
    isomorphism inductively.
  \end{proof}
The vanishing groups can also be handled directly.
\begin{proposition}
  For $n \neq m$, have $H^n(\mathbb{S}^m,G) \cong \mathbbm{1}$.
\end{proposition}
\begin{proof}
  Let us first consider the case $n > m$. Since $K(G,n)$ is
  $n$-truncated, we have $K(G,n) \simeq \truncT{K(G,n)}_n$. We induct
  on $m$ and when $m = 0$, we have
  \begin{align*}
    H^n(\mathbb{S}^0) = \truncT{\mathbb{S}^0 \to K(G,n)}_0 \simeq \truncT{K(G,n) \times K(G,n)}_0
  \end{align*}
  which vanishes since $K(G,n)$ is $(n-1)$-connected and $n > 0$. For
  larger $m$, we know by suspension that $H^n(\mathbb{S}^m) \cong
  H^{n-1}(\mathbb{S}^{m-1})$ which vanishes by the induction
  hypothesis.

  We give a similar proof when $n<m$. This time, we induct on
  $n$ and when $n = 0$, we have
  %
  \begin{align*}
    H^0(\mathbb{S}^m) = \truncT{\mathbb{S}^m \to G}_0
  \end{align*}
  %
  which vanishes because there are no non-trivial from $\mathbb{S}^m$
  into a set when $m > 0$. The induction step is, like in the first
  half of this proof, completed by applying the suspension
  isomorphism.
\end{proof}

Having computed these groups the cohomology ring of the spheres is
easily computed.

\begin{proposition}\label{prop:H*-Sn}
    Given any ring $R$ and $n \geq 1$, we have
    $H^*(\mathbb{S}^n,R) \cong R[x]/(x^2)$.
  \end{proposition}
\begin{proof}
  The only non-trivial cohomology groups are
  $H^0(\mathbb{S}^n,R) \cong H^n(\mathbb{S}^n,R) \cong R$. Thus, the
  cup product can only be non-trivial in dimensions $0 \times n$ and
  $n \times 0$. In these dimension, the cup product is simply left
  respectively right $R$-multiplication. This gives the desired
  isomorphism by letting constants in $H^*(\mathbb{S}^n,R)$ represent
  elements coming from $H^0(\mathbb{S}^n,R)$ and elements of degree
  one represent elements coming from $H^n(\mathbb{S}^n,R)$.
\end{proof}

\subsection{The Real Projective Plane and The Klein Bottle}

Let us consider two more complex, but closely related, examples: the
cohomology of the real projective plane and the Klein bottle. In HoTT,
we define the real projective plane, $\mathbb{R}P^2$, and the Klein
bottle, $K^2$, by HITs corresponding to their usual folding diagrams.
\begin{definition}[The real project plane]\label{def:RP2}
  We define $\mathbb{R}P^2$ as the HIT generated by the following constructors:\\
\begin{minipage}{.46\textwidth}
\begin{itemize}
\item $\star : \mathbb{R}P^2$
\item $\ell : \star = \star$
\item $\mathsf{sq} : \ell^{-1} = \ell$, i.e.\ a filler of the square:
\end{itemize}
\end{minipage}
\begin{minipage}{.54\textwidth}
\[\begin{tikzcd}[ampersand replacement=\&]
	\star \& \star \\
	\star \& \star
	\arrow["\ell",from=2-2,to=2-1]  %\arrow[Rightarrow, no head, from=2-1, to=2-2]
        \arrow["\ell",from=1-1,to=1-2]  %\arrow[Rightarrow, no head, from=2-1, to=2-2]
	\arrow[Rightarrow, no head, from=2-2, to=1-2]
	\arrow[Rightarrow, no head, from=1-1, to=2-1]
\end{tikzcd}\]
\end{minipage}
\end{definition}
\begin{definition}[The Klein bottle]\label{def:K2}
  We define $K^2$ as the HIT generated by the following
  constructors:\linebreak
  \begin{minipage}{.65\textwidth}
  \begin{itemize}
  \item $\star : K^2$
  \item $\ell_1,\ell_2 : \star = \star$
  \item $\mathsf{sq} : \Square{l_2}{l_2}{l_1^{-1}}{l_1}$, i.e.\ a filler of the
    square:
  \end{itemize}
  \end{minipage}
  \begin{minipage}{.39\textwidth}
    \begin{tikzcd}[ampersand replacement=\&]
	\star \& \star \\
	\star \& \star
	\arrow["{\ell_2}", from=1-1, to=1-2]
	\arrow["{\ell_2}"', from=2-1, to=2-2]
	\arrow["{\ell_1}"', from=2-2, to=1-2]
	\arrow["{\ell_1}"', from=1-1, to=2-1]
    \end{tikzcd}
  \end{minipage}
\end{definition}

Let us first tackle the cohomology of $\mathbb{R}P^2$. It is an easy
lemma that $\RP$ is $0$-connected, and hence $H^0(\RP,G) \cong G$. In
order to compute the higher cohomology groups, we will need to
introduce some new constructions; for an abelian group $G$ and an
integer $n \geq 0$, let $G[n]$ denote $n$-torsion subgroup of $G$,
i.e.\ the kernel of the map $n \cdot (-) : G \to G$. Let $G/n$ denote
the cokernel of the same homomorphism; that is, the group $G/\sim$
where $\sim$ is the relation $x^n = 0$.  We denote the quotient map
$G \to G/n$ by $[-]$.
\begin{proposition}\label{prop:H1-RP2}
  $H^1(\mathbb{R}P^2,G) \cong G[2]$
\end{proposition}
\begin{proof}
  The elimination principle for $\RP$ tells us that
  \[(\RP \to G) \simeq \sum_{x : K(G,1)}\sum_{p : x = x} (p^{-1} = p) \simeq \sum_{x : K(G,1)}\sum_{p : x = x} (p \cdot p = \refl) \]
  Since $K(G,n)$ is homogeneous this is equivalent to the following type
  \[{K(G,1)} \times \sum_{p : \Omega K(G,1)} (p \cdot p = \refl) \]
  which under the equivalence $\Omega K(G,1) \simeq G$ is equivalent
  to the type
  \[{K(G,1)} \times \sum_{g : G} (g + g = 0_G) = K(G,1) \times G[2] \]
  Thus, we get
\begin{align*}
  H^1(\RP,G) = \truncT{\RP \to K(G,1)}_0 &\simeq \truncT{K(G,1) \times G[2] }_0 \\
  &\simeq \truncT{K(G,1)}_0 \times G[2] \\
  &\simeq G[2]
\end{align*}
We verify that the inverse of this equivalence is a homomorphism. The
inverse $\psi : G[2] \to H^1(\RP,G)$ is given by $\psi(g) = f_g$ where
$f_g : \RP \to K(G,1)$ sends $\star$ to $0_k$ and $\ell$ to
$\LoopG{g}$. We do not need to worry about its action on $\mathsf{sq}$:
for truncation reasons this is not data but a property. We need to
verify that $f_{g_1+g_2}(x) = f_{g_1}(x) +_k f_{g_2}(x)$ for $x : \RP$
and $g_1,g_2 : G$. When $x$ is $\star$, this holds by $\refl$. For the
action on $\ell$, we need to verify that
\begin{align*}
  \LoopG{(g_1+g_2)} = \app{+_k}{\LoopG{g_1}}{\LoopG{g_2}}
\end{align*}
which we already verified in the proof of Proposition
\ref{prop:H1-S1}. This concludes the proof.
\end{proof}

\begin{proposition}\label{prop:H2-RP2}
  $H^2(\RP,G) \cong G/2$
\end{proposition}
\begin{proof}
  \todo{Väldigt mycket ``we... we... we...'' i det här beviset. Kan
    det formuleras om så att det är lite trevligare att läsa?}  Like
  in the proof of Proposition \ref{prop:H1-RP2}, we have
  \begin{align*}
    (\RP \to K(G,2)) &\simeq \sum_{x : K(G,2)}\sum_{p : x = x} {p \cdot p = \refl} \\
    &\simeq K(G,2) \times \sum_{p : \Omega K(G,2)} {p \cdot p = \refl} \\
    &\simeq K(G,2) \times \sum_{x : K(G,1)}{x +_k x = 0_k}
  \end{align*}
  Under set truncation, the $K(G,2)$-component vanishes and we are
  left with the type $\truncT{\sum_{x : K(G,1)}{x +_k x = 0_k}}_0$. Let us
  construct a map $\phi : \truncT{\sum_{x : K(G,1)}{x +_k x = 0_k}}_0 \to G/2$ by means
  of a curried map $\phi_x : x +_k x = 0_k \to G/2$ depending on
  $x : K(G,1)$. We may define it by the set-elimination rule for
  $K(G,1)$. When $x$ is $0_k$, want a map
  $\phi_{\star} : \Omega K(G,1) \to G/2$ which we can get by
  $\phi_{\star} := [-] \circ \sigma_0^{-1}$. We now need to describe
  the action on $\LoopG{g}$. This amounts to providing a path
  $[g] = [g' + g + g']$, which we of course have in $G/2$. Thus, we may define $\phi(\trunc{x,p}) := \phi_x(p)$

  We define the
  inverse
  $\psi : G/2 \to \truncT{\Sigma_{x : K(G,1)} (x+_k x = 0_k)}_0$ on
  canonical elements by $\psi[g] = (0_k,\LoopG{g})$. In order to show
  that this is well-defined, we need to show that
\begin{align*}
  \trunc{(0_k, \refl)} = \trunc{(0_k,\LoopG{(g+_G g)})}
\end{align*}
We do this component-wise. First, we need a path $0_k = 0_k$. For
this, we do \emph{not} choose $\refl$. Instead, we provide
$\LoopG{g}$. In order to show that the second components agree,
amounts to providing a filler of the square
\[\begin{tikzcd}[ampersand replacement=\&]
	{0_k} \&\& {0_k} \\
	\\
	{0_k} \&\& {0_k}
	\arrow["{\LoopG{(g+_G g)}}", from=1-1, to=1-3]
	\arrow["({\app{+_k}{\LoopG{g}}{\LoopG{g}})^{-1}}", from=3-1, to=1-1]
	\arrow["{\mathsf{refl}}"', Rightarrow, no head, from=3-1, to=3-3]
	\arrow["{\mathsf{refl}}"', Rightarrow, no head, from=3-3, to=1-3]
\end{tikzcd}\]
which is equivalent to proving that $\LoopG{(g +_G g)} =
\app{+_k}{\LoopG{g}}{\LoopG{g}}$, which we have already done in~the proofs of~Propositions~\ref{prop:H1-S1}~and~\ref{prop:H1-RP2}.

Finally, we prove that the maps cancel. Verifying that $\phi(\psi(x) =
x$ for $x:G/2$ is very direct: since the statement is a proposition,
it suffices to to this when $x$ is on the form $[g]$. In this case, we
have $\phi(\psi[g]) := \phi_{0_k}(\LoopG{g}) :=
\sigma_0^{-1}(\sigma_0(g)) = g$.

For the other direction, the fact that we are proposition
means that it suffices to show the cancellation it for elements of
$\truncT{\Sigma_{x : K(G,1)} (x +_k x = 0_k)}_0$ on the
form $\trunc{(0_k,p)}$ with $p : \Omega K(G,1)$. We get
$\psi(\phi\,\trunc{0_k,p}) := \psi(\sigma_0^{-1}(p)) = \trunc{0_k,\sigma_0(\sigma_0^{-1}(p)) = \trunc{0_k,p}}$.
Thus, we have shown:
\begin{align*}
H^2(\RP,G) &\simeq \bigg\Vert K(G,2) \times \sum_{x : K(G,1)}{x +_k x = 0_k} \bigg\Vert_0 \\
&\simeq \bigg\Vert \sum_{x : K(G,1)}{x +_k x = 0_k} \bigg\Vert_0\\
&\simeq G/2
\end{align*}
The argument for why this equivalence is a homomorphism is similar to
the argument given in previous proofs.
\end{proof}

\begin{proposition}\label{prop:H-high-RP2}
  $H^n(\RP,G)$ is trivial for $n > 2$.
\end{proposition}
\begin{proof}
  As we have seen in the two previous proofs:
  \begin{align*}
    H^n(\RP,G) &\simeq \bigg\Vert K(G,n) \times \sum_{x : K(G,n-1)} x +_k x = 0_k \bigg\Vert_0 \\
    &\simeq \bigg\Vert \sum_{x : K(G,n-1)} x +_k x = 0_k \bigg\Vert_0
  \end{align*}
  We may move in the truncation one step further to get
  \begin{align*}
    \bigg\Vert \sum_{x : K(G,n-1)} \truncT{x +_k x = 0_k}_0\bigg\Vert_0
  \end{align*}
  Since $n > 2$, any path space over $K(G,n-1)$ is (at least)
  $0$-connected. Thus, the truncation kills the space $(x +_k x =
  0_k)$. Hence, the above type is simply $\truncT{K(G,n-1)}_0$, which
  also vanishes due to connectedness.
\end{proof}

This gives us all the cohomology groups of $\RP$. We will now see how
this, in a rather direct way, gives us all the cohomology groups of
$K^2$ as well. Trivially, $H^0(K^2,G) \cong G$ for connectedness
reasons.

\begin{proposition}\label{prop:Hn-K2}
  $H^n(K^2,G) \cong \begin{cases} H^n(\RP,G) & n \neq 1 \\ G \times H^1(\RP,G) & n = 1 \end{cases}$
\end{proposition}
\begin{proof}
  Consider the mapping space $(K^2 \to K(G,n))$:
  \begin{align*}
    (K^2 \to K(G,n)) \simeq \sum_{x : K(G,n)}\sum_{p,q: x = x}(p
    \cdot q \cdot p = q)
  \end{align*}
  Again, we may use homogeneity of $K(G,n)$ to show that this is
  equivalent to the type $K(G,n) \times \sum_{p,q: \Omega K(G,n)}(p
  \cdot q \cdot p = q)$. We now consider the path space $p \cdot q
  \cdot p = q$ for $p,q : \Omega K(G,n)$. By commutativity of
  $\Omega\,K(G,n)$, composing both sides by $q^{-1}$ will cancel out
  $q$ everywhere. Thus, the type is simply $p\cdot p = \refl$. Hence, we have
  \begin{align*}
    H^n(K^2,G) &:= \truncT{K^2 \to K(G,n)}_0 \\
               &\simeq \bigg\Vert K(G,n) \times \Omega K(G,n) \times \sum_{p : \Omega K(G,n)} (p \cdot p \equiv \refl)\bigg\Vert_0
  \end{align*}
%
  Excluding the $\Omega K(G,n)$ component, this is precisely the
  characterisation of $H^n(\RP,G)$. Thus, the above type is equivalent
  to
  \begin{align*}
    \truncT{\Omega K(G,n)}_0 \times H^n(\RP,G)
  \end{align*}
  The factor $\truncT{\Omega K(G,n)}_0$ vanishes for $n \neq 1$. When
  $n = 1$, we have $\truncT{\Omega K(G,1)}_0 \simeq \truncT{G}_0
  \simeq G$. Verifying that this is a homomorphism is straightforward
  but somewhat technical.
\end{proof}

Computing the integral cohomology ring of $\RP$ is straightforward.
Naturally, the below proposition easily generalises to $H^*(\RP,R)$
for any $2$-torsion free ring $R$.

\begin{proposition}
  $H^*(\RP,\bZ) \cong \bZ[x]/(2x,x^2)$
\end{proposition}
\begin{proof}
  By Proposition \ref{prop:H1-RP2}, we have
  $H^1(\RP,\bZ) \cong \bZ[2]$. Since $\bZ$ has no non-trivial torsion
  elements, this tells us that $H^1(\RP,\bZ)$ is trivial. Hence, we
  only have as non-trivial cohomology groups the groups
  $H^0(\RP,\bZ) \cong \bZ$ and $H^2(\RP,\bZ) \cong \bZTwo$. The proof
  now proceeds just like that of Proposition \ref{prop:H*-Sn},
  representing elements from $H^0(\RP,\bZ)$ and elements from
  $H^2(\RP,\bZ)$ respectively by degree-$0$ and degree-$1$ elements in
  $H^*(\RP,\bZ)$. The $2x$-quotient comes from the $2$-torsion in
  $H^2(\RP,\bZ)$.
\end{proof}

Let us now turn to the Klein bottle. For the coming results, the
following construction will be crucial.
\begin{definition}
  There is a homotopy
  $$\killDiag : (p : \Omega K(G,n))  \to  \app{\smile_k}{p}{p} = 0_k$$
  defined by the composite path
\[\begin{tikzcd}[ampersand replacement=\&]
	{\mathsf{ap}^2_{\smile_k}(p,p)} \&\&\& {\mathsf{ap}_{(-)\smile_k 0_k}(p)\cdot \mathsf{ap}_{0_k\smile_k (-)}(p)} \&\& \refl
	\arrow["{h(p)}", from=1-4, to=1-6]
	\arrow["{\textsf{ap}_{\smile_k}^2\textsf{-funct}(p,p)}", from=1-1, to=1-4]
      \end{tikzcd}\]
    Here $h(p)$ is given by pointwise application of the right and
    left annihilation laws for $\smile_k$ using that they agree on
    $0_k$.
\end{definition}

We will rely on this construction to kill of certain cup products on
\RP and $K^2$. For instance, it makes the following computation easy.
%\anders{Samma kommentar om att detta generalizerar till 2-torsion-fria
%  ringar gäller här va? --- Inte säker på att det är lika självklart}

\begin{proposition}
  $H^*(K^2,\bZ) \cong \bZ[x,y]/(2y,x^2,y^2,xy)$
\end{proposition}
\begin{proof}
  \anders{Kolla igenom det här beviset igen sen}

  Using Proposition \ref{prop:Hn-K2} and the preceeding results, we know that the
  only non-trivial cohomology groups of $K^2$ are
  \begin{align*}
    H^0(K^2,\bZ) &\cong \bZ \\
    H^1(K^2,\bZ) &\cong \bZ \times \bZ[2] \cong \bZ \\
    H^2(K^2,\bZ) & \cong \bZTwo
  \end{align*}
  Consider first the ring $\bZ[x,y]$. Using the above isomorphisms, we
  may naively let degree-$0$ elements in $\bZ[x,y]$ represent elements
  from $H^0(K^2,\bZ)$, degree $1$ elements with $x$-term represent
  elements from $H^1(K^2,\bZ)$ and degree-$1$ elements represent
  elements from $H^2(K^2 ,\bZ)$. Under this identitifcation, we see
  that the relations described by the ideal $(2y,xy,y^2)$ are
  satisfied. Hence, we have a map $bZ[x,y]/(2y,xy,y^2) \to
  H^1(K^2,\bZ)$.  In order to lift this to an isomorphism
  $\bZ[x,y]/(2y,x^2,y^2,xy) \cong H^*(K^2,\bZ)$, we need to show that
  the cup product is trivial in dimension $1 \times 1$. It suffices to
  show that it vanishes on generators. We can easily define a map
  $\alpha : K^2 \to K(1,\mathbb{Z})$ such that $\trunc{\alpha}$
  generates $H^1(K^2,\bZ)$. We define it by
\begin{align*}
  \alpha(\star) &= 0_k \\
  \ap{\alpha}{\ell_1} &= \refl \\
  \ap{\alpha}{\ell_2} &= \LoopG{1}
\end{align*}
where, $1 : \bZTwo$ denotes the generator. The final step of the
definition, i.e.\ the action of $\alpha$ on $\mathsf{sq}$, corresponds
to providing a proof that $\LoopG{1} = \LoopG{1}$, which we do by
$\refl$. Let $x : K^2$. We show that $\alpha(x) \smile_k \alpha(x) =
0_k$ by induction on $x$. We prove $\alpha(\star) = 0_k $ by $\refl$
and $\ap{\alpha}{\ell_2} = \refl$ by $\refl$. For
$\ap{\alpha}{\ell_1}$, we need to provide a path
$\app{\smile_k}{\LoopG{1}}{\LoopG{1}} = \refl$, which we give by
$\killDiag(\LoopG{1})$. Finally, for the action of $\mathsf{sq}$, we
need to provide a filler of the square
\[\begin{tikzcd}[ampersand replacement=\&]
	{\app{\smile_k}{\LoopG{1}}{\LoopG{1}}} \&\& {\refl} \\
	\\
	{\app{\smile_k}{\LoopG{1}}{\LoopG{1}}} \&\& {\refl}
	\arrow["{\killDiag(\LoopG{1})}", from=1-1, to=1-3]
	\arrow["{\mathsf{refl}}"', Rightarrow, no head, from=1-1, to=3-1]
	\arrow["{\killDiag(\LoopG{1})}"', from=3-1, to=3-3]
	\arrow["{\mathsf{refl}}"', Rightarrow, no head, from=3-3, to=1-3]
\end{tikzcd}\]
which is trivial. Thus, we have shown, in particular, that
$\trunc{\alpha} \smile \trunc{\alpha}$ is trivial, which means that
$\smile$ vanishes everywhere in dimension $1 \times 1$. This concludes
the proof.
\end{proof}
Let us now turn to the $\bZTwo$-cohomology of $K^2$ and \RP. When
working in $\bZTwo$-coefficients, it turns out that we will need to
investigate $\killDiag$ further. In particular, it turns out that
applying $\killDiag$ may give rise to non-trivial homotopies. In
particular, the twist in \RP and $K^2$ will force us to investigate
how much $\killDiag$ commutes with path inversion in the sense that
there exists a loop $q : \Omega^2 K(\bZTwo,2n)$ solving the following
square filling problem
\[\begin{tikzcd}[ampersand replacement=\&]
	{\mathsf{ap}^2_{\smile_k}(p,p)} \&\&\& \refl \\
	{(\mathsf{ap}^2_{\smile_k}(p^{-1},p^{-1}))^{-1}} \&\&\& \refl
	\arrow[from=1-1, to=2-1]
	\arrow["{\ap{(-)^{-1}}{\killDiag(p^{-1})}}"', from=2-1, to=2-4]
	\arrow["{\killDiag(p)}", from=1-1, to=1-4]
	\arrow["q", dashed, from=1-4, to=2-4]
\end{tikzcd}\]
We remark that the only case of interest to us is the case $n = 1$, due to the
vanishing of higher homotopy groups. In order to do this, we will need
the following construction.


%% \begin{lemma}
%%   Given pointed types $A$ and $B$ and a binary function $F : A \to A
%%   \to B$ equippied with homotopies $F_l : (x : A) \to F(x,\star_A) =
%%   \star_B$ and $F_r : (y : A) \to F(\star_a,y)$ and a coherence
%%   $fF_{lr} : F_l(\star_A) = F_R(\star_A)$, there is, for every $p : \Omega\,A$ a filler of the square \[\begin{tikzcd}[ampersand replacement=\&]
%% 	{\star_B} \&\& {\star_B} \\
%% 	\\
%% 	{F(\star_A,\star_A)} \&\& {F(\star_A,\star_A)}
%% 	\arrow["{F_l(\star_A)}", from=3-1, to=1-1]
%% 	\arrow[""{name=0, anchor=center, inner sep=0}, "{\mathsf{ap}^2_{F}(p,p)}"', from=3-1, to=3-3]
%% 	\arrow["{F_l(\star_A)}"', from=3-3, to=1-3]
%% 	\arrow[""{name=1, anchor=center, inner sep=0}, "\refl", from=1-1, to=1-3]
%% 	\arrow["{\killDiagGen_F(p)}"{description}, shorten <=9pt, shorten >=9pt, Rightarrow, from=0, to=1]
%% \end{tikzcd}\]
%% \end{lemma}
%% \begin{proof}
%%   The homotopy is given by as the outer square of the following composition
%% \[\begin{tikzcd}[ampersand replacement=\&]
%% 	{\star_B} \&\&\& {\star_B} \& {} \& {\star_B} \\
%% 	\\
%% 	{F(\star_A,\star_A)} \&\&\& {F(\star_A,\star_A)} \& {} \& {F(\star_A,\star_A)} \\
%% 	{F(\star_A,\star_A)} \&\&\&\&\& {F(\star_A,\star_A)} \\
%% 	{F(\star_A,\star_A)} \&\&\&\&\& {F(\star_A,\star_A)}
%% 	\arrow[""{name=0, anchor=center, inner sep=0}, "{F_r(\star_A)}"{description}, bend right ={60}, from=3-4, to=1-4]
%% 	\arrow[""{name=1, anchor=center, inner sep=0}, "{F_l(\star_A)}"{description}, bend left ={60}, from=3-4, to=1-4]
%% 	\arrow["{\mathsf{ap}_{F(-,\star_A)}(p)}"', from=3-4, to=3-6]
%% 	\arrow["\refl", from=1-4, to=1-6]
%% 	\arrow["{\mathsf{ap}_{F_l}(p)}"{description}, shorten <=3pt, shorten >=3pt, Rightarrow, from=3-5, to=1-5]
%% 	\arrow["{F_l(\star_A)}"', from=3-6, to=1-6]
%% 	\arrow[""{name=2, anchor=center, inner sep=0}, "{\mathsf{ap}_{F(\star_A,-)}(p)}"', from=3-1, to=3-4]
%% 	\arrow[""{name=3, anchor=center, inner sep=0}, "\refl", from=1-1, to=1-4]
%% 	\arrow[""{name=4, anchor=center, inner sep=0}, "{F_r(\star_A)}"{description}, bend right ={60}, from=3-1, to=1-1]
%% 	\arrow[""{name=5, anchor=center, inner sep=0}, "{F_l(\star_A)}"{description}, bend left ={60}, from=3-1, to=1-1]
%% 	\arrow["\refl"', from=4-6, to=3-6]
%% 	\arrow["\refl", from=4-1, to=3-1]
%% 	\arrow[""{name=6, anchor=center, inner sep=0}, "{\mathsf{ap}_{F(\star_A,-)}(p) \cdot \mathsf{ap}_{F(-,\star_A)}(p)}"{description}, from=4-1, to=4-6]
%% 	\arrow["\refl", from=5-1, to=4-1]
%% 	\arrow[""{name=7, anchor=center, inner sep=0}, "{\app{F}{p}{p}}"{description}, from=5-1, to=5-6]
%% 	\arrow["\refl"', from=5-6, to=4-6]
%% 	\arrow["{F_{l_r}^{-1}}"{description}, draw=none, from=0, to=1]
%% 	\arrow["{\mathsf{ap}_{F_r}(p)}"{description}, shorten <=9pt, shorten >=9pt, Rightarrow, from=2, to=3]
%% 	\arrow["{F_{l_r}}"{description}, draw=none, from=5, to=4]
%% 	\arrow["{\mathsf{ap}^2_F\textsf{-funct}(p)}"{description}, shorten <=4pt, shorten >=4pt, Rightarrow, from=7, to=6]
%% \end{tikzcd}\]
%% \end{proof}

\begin{definition}\label{def:res}
  Given two points $x ,y : A$ and a binary function function $f : A
  \to A \to B$, we construct the homotopy $$ \mathsf{Res}_F : (p : x = y) \to (\ap{F(-,y)}{p^{-1}} \cdot \ap{F(x,-)}{p^{-1}})^{-1} = \ap{F(-,x)}{p} \cdot \ap{F(y,-)}{p}$$ by the outer square of the following composite square
\[\begin{tikzcd}[ampersand replacement=\&]
	{F(x,x)} \&\&\&\&\&\& {F(y,y)} \\
	\\
	\& {F(x,x)} \&\&\&\& {F(y,x)} \\
	\\
	\& {F(x,y)} \&\&\&\& {F(y,y)} \\
	\\
	{F(x,x)} \&\&\&\&\&\& {F(y,y)}
	\arrow["{\mathsf{ap}_{F(y,-)}(p^{-1})}"{description}, from=5-6, to=3-6]
	\arrow["\refl"{description}, from=7-1, to=1-1]
	\arrow["\refl"{description}, from=3-2, to=1-1]
	\arrow["{\mathsf{ap}_{F(x,-)}(p^{-1})}"{description}, from=5-2, to=3-2]
	\arrow["{(\mathsf{ap}_{F(x,-)}(p^{-1}))^{-1}}"{description}, from=5-2, to=7-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\mathsf{ap}_{F(-,y)}(p)}"', from=5-2, to=5-6]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\mathsf{ap}_{F(-,x)}(p)}", from=3-2, to=3-6]
	\arrow["{\mathsf{ap}_{F(y,-)}(p)}"{description}, from=3-6, to=1-7]
	\arrow["{\mathsf{ap}_{F(-,x)}(p) \cdot \mathsf{ap}_{F(y,-)}(p)}"{description}, from=1-1, to=1-7]
	\arrow["{(\mathsf{ap}_{F(-,y)}(p^{-1}) \cdot \mathsf{ap}_{F(x,-)}(p^{-1}))^{-1}}"{description}, from=7-1, to=7-7]
	\arrow["\refl"{description}, from=7-7, to=1-7]
	\arrow["\refl"{description}, from=5-6, to=7-7]
	\arrow["{\mathsf{ap}_{a \mapsto \mathsf{ap}_{F(-,a)}(p)}(p^{-1})}"{description}, shorten <=9pt, shorten >=9pt, Rightarrow, from=0, to=1]
\end{tikzcd}\]
where all the outermost squares are given by their obvious fillers. The crucial step is the bottom square.
\anders{Jag orkar inte dubbelkolla allt ovan nu, kan du göra det? -- Din tur;-)}
\end{definition}
The following lemma is immediate by path induction.
\begin{lemma}
  For any point $x: A$ and $F : A \to A \to B$, we have $\mathsf{Res}_F(\refl_{x}) = \refl$
\end{lemma}
The usefulness of $\mathsf{Res}$ is that it measures how much
$\mathsf{ap}^2_F\textsf{-funct}$ fails commute with path inversion, as
made clear by the following lemma.
\begin{lemma}\label{lem:res}
  Given a binary function $F : A \to A \to B$ and a path $p : x =_A y$, we have a filler
\[\begin{tikzcd}[ampersand replacement=\&]
	{\mathsf{ap}^2_F(p,p)} \&\&\&\& {\mathsf{ap}_{F(-,\star_A)}(p)\cdot \mathsf{ap}_{F(\star_A,-)}(p)} \\
	{(\mathsf{ap}^2_F(p^{-1},p^{-1}))^{-1}} \&\&\&\& {(\mathsf{ap}_{F(-,\star_A)}(p^{-1})\cdot \mathsf{ap}_{F(\star_A,-)}(p^{-1}))^{-1}}
	\arrow[from=1-1, to=2-1]
	\arrow["{\mathsf{Res}_F(p)}", from=1-5, to=2-5]
	\arrow["{\textsf{ap}_F^2\textsf{-funct}(p,p)}", from=1-1, to=1-5]
	\arrow["{\mathsf{ap}_{(-)^{-1}}(\textsf{ap}_F^2\textsf{-funct}(p^{-1},p^{-1}))}"', from=2-1, to=2-5]
\end{tikzcd}\]
where the left-most path is the obvious coherence (defined by path induction in Book HoTT and simply by $\refl$ in cubical type theory).
\end{lemma}
\begin{proof}
  Path induction on $p$.
\end{proof}

What is rather surprising is that $\mathsf{Res}_F(p)$ is not just a
mere coherence path: it may be homotopically non-trivial when $p$ is a
loop. In particular, when $p$ is $\LoopG{1} : \Omega K(G,1)$ and $F$ is
the cup product $\smile_k : K(\bZTwo,1) \to K(\bZTwo,1) \to
K(\bZTwo,2)$, the inner square in Definition \ref{def:res} is, modulo
cancellation laws, precisely the two-cell $\sigma^2(1) :
\Omega^2 K(\bZTwo,2)$ (here $\sigma^2$ is shorthand for $\mathsf{ap}_{\sigma_1}\circ \sigma_0 : K(\bZTwo,0) \to \Omega^2 K(\bZTwo,2)$). This follows directly by construction of the cup
product. Hence we arrive at the following lemma, which is key to analysing  the behavour of the cup product on $\RP$ and $K^2$.
\begin{lemma}\label{lem:killDiag-comm}
  We have a filler of the following square
\[\begin{tikzcd}[ampersand replacement=\&]
	{\mathsf{ap}^2_{\smile_k}(\LoopG{1},\LoopG{1})} \&\&\& \refl \\
	{(\mathsf{ap}^2_{\smile_k}((\LoopG{1})^{-1},(\LoopG{1})^{-1}))^{-1}} \&\&\& \refl
	\arrow[from=1-1, to=2-1]
	\arrow["{\ap{(-)^{-1}}{\killDiag({\LoopG{1}}^{-1})}}"', from=2-1, to=2-4]
	\arrow["{\killDiag(\LoopG{1})}", from=1-1, to=1-4]
	\arrow["{\sigma^2(1)}", from=1-4, to=2-4]
\end{tikzcd}\]
\end{lemma}
We may now characterise the cup product on the cohomology groups of
$\RP$ and $K^2$ with $\mathbb{Z}/2\mathbb{Z}$ coefficients. In fact,
Lemma \ref{lem:killDiag-comm} is the only technical lemma we will
need, and we do not need to rely on any other advanced
theorems/constructions. Let us start with $\RP$.
\begin{proposition}\label{prop:RP-cup}
  The follow diagram commutes
\[\begin{tikzcd}[ampersand replacement=\&]
	{\bZTwo \times \bZTwo} \& {\bZTwo} \\
	{H^1(\RP,\bZTwo) \times H^1(\RP,\bZTwo)} \& {H^2(\RP,\bZTwo)}
	\arrow["\smile", from=2-1, to=2-2]
	\arrow["\sim", sloped, from=1-1, to=2-1]
	\arrow["{\mathsf{mult}}", from=1-1, to=1-2]
	\arrow["\sim", sloped, from=1-2, to=2-2]
\end{tikzcd}\]
\end{proposition}
\begin{proof}
  \anders{Kolla igenom det här beviset igen}

  It is enough to show that $\trunc{\alpha} \smile \trunc{\alpha} =
  \trunc{\beta}$ for generators $\alpha : \RP \to K(\bZTwo,1)$ and
  $\beta : \RP \to K(\bZTwo,2)$. We define $\alpha$ by
  \begin{align*}
    \alpha(\star) &= 0_k \\
    \ap{\alpha}{\ell} &= \LoopG{1} \\
    \ap{\mathsf{ap}_{\alpha}}{\mathsf{sq}} &= Q(\LoopG{1})
  \end{align*}
  where $Q : (p : \Omega\,K(\bZTwo,1) \to p = p^{-1}$ is given
  by the $2$-torsion in $K(\bZTwo,n)$ (its explicit construction is
  irrelevant for our purposes). We define $\beta$ by
  \begin{align*}
    \alpha(\beta) &= 0_k \\
    \ap{\beta}{\ell} &= \refl \\
    \ap{\mathsf{ap}_{\beta}}{\mathsf{sq}} &= \sigma^2(1)
  \end{align*}
  where $\sigma^2 : \bZTwo \xrightarrow{\sim} \Omega^2 K(\bZTwo,2)$. The fact
  that $\alpha$ and $\beta$ define generators on cohomology is
  straightforward by the constructions in the proofs of Propositions
  \ref{prop:H1-RP2} and \ref{prop:H2-RP2}. We now provide a homotopy
  $h : (x : \RP) \to \alpha(x) \smile_k\alpha(x) = \beta(x)$. We
  define
  \begin{align*}
    h(\star) &= \refl\\
    \ap{h}{\ell} &= \killDiag(\LoopG{1})
  \end{align*}
  For the action of $h$ on $\mathsf{sq}$, we need to provide a filler
  of the following square of paths.
\[\begin{tikzcd}[ampersand replacement=\&]
	{\mathsf{refl}} \&\&\&\& {\mathsf{refl}} \\
	\\
	\\
	{\mathsf{ap}_{\smile_k}^2(\LoopG{1},\LoopG{1})} \&\&\&\& {\mathsf{ap}^2_{\smile_k}(\LoopG{1},\LoopG{1})^{-1}}
	\arrow["{\sigma^{2}(1)}", from=1-1, to=1-5]
	\arrow["{\killDiag(\LoopG{1})}", from=4-1, to=1-1]
	\arrow["{\mathsf{ap}_{\mathsf{ap}_{\smile_k \circ \Delta}}(Q(\LoopG{1}))}"', from=4-1, to=4-5]
	\arrow["{\mathsf{ap}_{(-)^{-1}}(\killDiag(\LoopG{1}))}"', from=4-5, to=1-5]
\end{tikzcd}\]
The bottom path acts on the right-hand path by moving in a path inversion around $\LoopG{1}$. Hence, our new square filling problem is
\[\begin{tikzcd}[ampersand replacement=\&]
	{\mathsf{refl}} \&\&\&\& {\mathsf{refl}} \\
	\\
	\\
	{\mathsf{ap}_{\smile_k}^2(\LoopG{1},\LoopG{1})} \&\&\&\& {\mathsf{ap}^2_{\smile_k}((\LoopG{1})^{-1},(\LoopG{1})^{-1})^{-1}}
	\arrow["{\sigma^{2}(1)}", from=1-1, to=1-5]
	\arrow["{\killDiag(\LoopG{1})}", from=4-1, to=1-1]
	\arrow[from=4-1, to=4-5]
	\arrow["{\mathsf{ap}_{(-)^{-1}}(\killDiag((\LoopG{1})^{-1}))}"', from=4-5, to=1-5]
\end{tikzcd}\]
But this is precisely Lemma \ref{lem:killDiag-comm}, and we are done.
\end{proof}

As an immediate corollary, we get the cohomology ring of $\RP$ with
$\bZTwo$-coefficients. \todo{Kanske introducera notation $\bZ_2$ för
  $\bZTwo$ så blir polynomringen snyggare att skriva?}

\begin{proposition}
  $H^*(\RP,\bZTwo) \cong \bZTwo[x]/(x^3)$.
\end{proposition}
\begin{proof}
  We simply let elements in $H^n(\RP,\bZTwo)$ correspond to degree-$n$
  elements in $H^*(\RP,\bZTwo)$. By Proposition \ref{prop:RP-cup}, we
  know that the multiplicative structure on $H^*(\RP,\bZTwo)$ is
  regular $\bZTwo$-multiplcation, from which the statement follows.
\end{proof}

Let us now turn to the Klein bottle. Although the cohomology ring
structure is different, we may still make use of the above. We start
by considering its multiplicative structure. First, we construct the
generators $\alpha ,\beta : K^2 \to K(\bZTwo,1)$ by\newline
\begin{minipage}{.5\textwidth}
\begin{align*}
  \alpha(\star) &:= 0_k \\
  \ap{\alpha}{\ell_1} &:= \LoopG{1} \\
  \ap{\alpha}{\ell_2} &:= \refl \\
  \ap{\mathsf{ap}_\alpha}{\mathsf{sq}} &:= \mathsf{flip}(\refl_{\LoopG{1}})
\end{align*}
\end{minipage}
\begin{minipage}{.5\textwidth}
\begin{align*}
  \beta(\star) &:= 0_k \\
  \ap{\beta}{\ell_1} &:= \refl \\
  \ap{\beta}{\ell_2} &:= \LoopG{1} \\
  \ap{\mathsf{ap}_\beta}{\mathsf{sq}} &:= \refl_{\LoopG{1}}
\end{align*}
\end{minipage}
%
It is immediate by construction that the isomorphism
$H^1(K^2,\bZTwo) \cong \bZTwo \times \bZTwo$ takes $\trunc{\alpha}$ to
$(1,0)$ and $\trunc{\beta}$ to $(0,1)$. The single generator of
$H^2(K^2,\bZTwo)$ is given by $\gamma : K^2 \to K(\bZTwo,2)$:
\begin{align*}
  \gamma(\star) &:= 0_k \\
  \ap{\gamma}{\ell_1} &:= \refl \\
  \ap{\gamma}{\ell_2} &:= \refl \\
  \ap{\mathsf{ap}_\gamma}{\mathsf{sq}} &:= \sigma^2(1)
\end{align*}
It again follows by construction that the isomorphism
$H^2(K^2,\bZTwo) \cong \bZTwo$ takes $\trunc{\gamma}$ to $1$.
\begin{proposition}\label{prop:H*-K2-rels}
  We have the following relations in $H^*(K^2,\bZTwo)$
  \begin{align*}
    \trunc{\alpha}^2 = \gamma \hspace{3cm} \trunc{\alpha} \smile \trunc{\beta} = \gamma \hspace{3cm} \trunc{\beta}^2 = 0_h
  \end{align*}.
\end{proposition}
\begin{proof}
  Let us deal with the identities from right to left, in increasing
  difficulty. Showing that $\beta^2 = 0_h$ is easy. First construct a
  homotopy $f : (x : K^2) \to \beta(x) \smile_k \beta(x) = 0_k$ by
  induction on $x$.
  \begin{align*}
    f(\star) &:= \refl \\
    \ap{f}{\ell_1} &:= \refl \\
    \ap{f}{\ell_2} &:= \killDiag(\LoopG{1})
  \end{align*}
  For the action on $\mathsf{sq}$, we are reduced to simply providing
  a path $\killDiag(\LoopG{1}) = \killDiag(\LoopG{1})$, which we can by
  $\refl$. This gives us, in particular, that $\trunc{\beta}^2 = 0_h$.

  Let us now provide a homotopy $g : (x : K^2) \to \alpha(x) \smile_k
  \beta(x) = \gamma(x)$. We again proceed by $K^2$-induction.
  \begin{align*}
    g(\star) &:= \refl \\
    \ap{g}{\ell_1} &:= \refl \\
    \ap{g}{\ell_2} &:= \refl
  \end{align*}
The reason that $\refl$ works for the action on $\ell_1$ and $\ell_2$
is because $\ap{0_k \smile_k (-)}{\LoopG{1}}$ and $\ap{(-) \smile_k
  0_k}{\LoopG{1}}$ by definition reduce to $\refl_{0_k}$. The final step amount to showing that
\begin{align*}
  \ap{x \mapsto \ap{y \mapsto \alpha(x) \smile_k
      \beta(y)}{\LoopG{1}}}{\LoopG{1}} = \sigma^2(1)
\end{align*}
which is easy to see by unfolding the definition of $\smile_k$. Thus,
we have $\trunc{\alpha} \smile \trunc{\beta} = \trunc{\gamma}$.

Finally, let us verify that $\trunc{\alpha}^2 = \trunc{\gamma}$. We
construct a homotopy $h : (x : K^2) \to \alpha(x) \smile_k \alpha(x) =
\gamma(x)$ by
  \begin{align*}
    h(\star) &:= \refl \\
    \ap{h}{\ell_1} &:= \killDiag(\LoopG{1}) \\
    \ap{h}{\ell_2} &:= \refl
  \end{align*}
  For the action on $\mathsf{sq}$, we end up having to fill another
  square (or rather: another degenerate cube); fortunately for us,
  this filling problem can easily be reduced to that of filling the
  first square appearing in the proof of
  Proposition~\ref{prop:RP-cup}, which we have already filled. Thus
  $\trunc{\alpha}^2 = \trunc{\gamma}$.
\end{proof}
\begin{corollary} %% <X³,Y²,XY+X²>
  $H^*(K^2,\bZTwo) \cong \bZTwo[x,y]/(x^3,y^2,xy+x^2)$
\end{corollary}
\begin{proof}
  By Proposition \ref{prop:H*-K2-rels}, we obtain the isomorphism by
  mapping the generators $1 : H^0(K^2,\bZTwo)$,
  $\alpha,\beta : H^1(K^2,\bZTwo)$ and $\gamma : H^2(K^2,\bZTwo)$ to
  $1$, $x$, $y$ and $x^2$ respectively.
\end{proof}

\subsection{The complex projective plane}
\label{sec:cp2}

Sometimes providing direct cohomology computations is rather
difficult. One example of a space whose cohomology is difficult to
compute directly, but is straightforward to compute using the Gysin
sequence is $\mathbb{C}P^2$, i.e.\ the cofibre of the Hopf
map $h : \mathbb{S}^{3} \to \mathbb{S}^{2}$, the details of which will
not be needed here (see \cite[Definition 5]{LICS23} for a
self-contained definition or \cite[Section 8.5]{HoTT13} for the
original definition in HoTT). This was first done in HoTT by
\citet{Brunerie16} who applied the Gysin sequence to the fibre
sequence
\begin{align}
  \label{eq:CP2seq}
  \mathbb{S}^1 \to \mathbb{S}^{5}\to \mathbb{C}P^2
\end{align}
It follows from the Mayer-Vietoris sequence that, for any group $G$,
the cohomology of $\mathbb{C}P^2$ is concentrated in degrees $0$, $2$
and $4$:
\begin{align*}
  H^m(\mathbb{C}P^n,G) \cong
  \begin{cases}
    G & \text{if $m \in \{0, n, 2n \}$} \\
    \mathbbm{1} & \text{otherwise}
    \end{cases}
\end{align*}
The space $\mathbb{C}P^2$ is $1$-connected and so we may apply the
Gysin sequence to \eqref{eq:CP2seq} with $n = 2$. Unfolding the
sequence for $i = 2$ and $i = 4$ tells us that
$e : H^2(\mathbb{C}P^2,\mathbb{Z})$ and
$e^2 : H^4(\mathbb{C}P^2,\mathbb{Z})$ are generators, thus giving us
$H^*(\mathbb{C}P^2,\mathbb{Z}) \cong \mathbb{Z}[x]/(x^3)$. This was
formalised in full detail in~\cite{CohomRings23}.

%\anders{Vad händer för godtycklig ring? --- Inte lika självklart. Man använder implicit att $\bZ$ har en unik (upp till ett teckenskifte) generator}

\subsection{Infinite projective space}
\label{sec:rpinf}

To further showcase the usefulness of the Gysin sequence, let us
compute $H^*(\RPinf,\bZ/2\bZ)$. This computation is particularly
interesting since it is an example of an application of the Gysin
sequence to a space which is \emph{not} $1$-connected. For it to work,
we hence need to construct the family $c_b$ in
\hyperref[gysin-cond]{($\ast$)}
explicitly. As $\RPinf$ is well-known
to be an Eilenberg-MacLane space we may conveniently define it by
$\RPinf := \KTwoOne$. We remark that this differs from the definition given in~\cite[Definition IV.1]{RPn}, but the argument we provide here should be easy to translate to fit their definition.
%% \todo{What's the oringal ref ref for this construction?} Following~\cite{?}, we define
%% \[\RPinf := \Sigma_{X : \mathsf{Type}} \truncT{X \simeq \mathbb{S}^0}_{-1}\]
%% Recall that $\mathbb{S}^0 := \mathsf{Bool}$ and we take it to be pointed by $\mathsf{true}$.
%% With some abuse of notation, we write $X : \RPinf$ for $X : \mathsf{Type}$ and take the element of $\truncT{X \simeq \mathbb{S}^0}_{-1}$ implicit. We t
%% Let us give an example of the Gysin sequence in action.
%% \todo{Check what is already proved about RPinf in other papers}
%% \begin{lemma}
%%   For $X : \RPinf$, we have that $X$ is a set.
%% \end{lemma}
%% \begin{proof}
%%   Since the statement that $X$ is a set is a proposition and $X$ is
%%   merely equivalent to $\mathbb{S}^0$, we may assume that $X$ is
%%   $\mathbb{S}^0$ which we know is a set.
%% \end{proof}
%% \begin{lemma}\label{lem:not-construction}
%%   For $X : \RPinf$, the type $\Sigma_{f : X \simeq X} (\neg (f = \mathsf{id}) \times (f \circ f = \mathsf{id}))$ is contractible.
%% \end{lemma}
%% \begin{proof}
%%   We are proving a proposition, so it suffices to prove it for $X := \mathbb{S}^0$. In this case, we are simply to prove that there is a unique non-identity involutive equivalence $\mathbb{S}^0 \simeq \mathbb{S}^0$. This is of course true, and is witnessed by the involution $\mathsf{not}_{\mathbb{S}^0} : \mathbb{S}^0 \to \mathbb{S}^0$.
%% \end{proof}
%% \begin{lemma}\label{lem:RPinf-paths}
%%   For $X : \RPinf$ the maps $\mathsf{from}^{\mathbb{S}^0\simeq} :
%%   \mathbb{S}^0 \simeq X \to X$ defined
%%   by $$\mathsf{from}^{\mathbb{S}^0\simeq}(e) := e(\mathsf{true})$$ is
%%   an equivalence.
%% \end{lemma}
%% \begin{proof}
%%   Again, we are proving a proposition, so it suffices to consider the cases when $X := \mathbb{S}^0$ in which case 
%% \end{proof}
%% \begin{corollary}
%%   The total space $\Sigma_{X : \RPinf} X$ is contractible.
%% \end{corollary}
%% \begin{proof}
%%   By~Lemma~\ref{lem:not-construction}, we have $X \simeq
%%   (\mathbb{S}^0 \simeq X)$. Applying univalence, we hence get $\Sigma_{X :
%%     \RPinf} X \simeq \Sigma_{X:\RPinf} (\mathbb{S}^0 = X)$ which is
%%   contractible.
%% \end{proof}
%% Lemma~\ref{lem:not-construction} gives us an involution $\mathsf{not}_X : X
%% \simeq X$ for each $X : \RPinf$. By construction, it is equal
%% to the usual involution on $\mathbb{S}^0$ when $X$ is $\mathbb{S}^0$.

Hence, we are to compute $H^*(\KTwoOne,\bZ/2\bZ)$. Using the
equivalence $\psi : \Omega \KTwoOne \simeq_\star \mathbb{S}^0$, we
construct the fibre sequence
\[\mathbb{S}^0 \to \Sigma_{x : \KTwoOne} (0_k = x) \to \KTwoOne\]
This fits the Gysin sequence with $n = 1$ and the fibration $P :
\KTwoOne \to \mathsf{Type}$ being defined by $P(x) := (0_k = x)$. In
order to apply the sequence, we need to construct, for each $x :
\KTwoOne$, a map
\[c_x : \Sigma (0_k = x) \to_\star K(\bZ/2\bZ,1)\] Let us initially
construct $c_x$ is the case when $x := 0_k$. In this case, the domain of $c_x$ is simply $\Sigma (\Omega(K(\bZTwo,1)))$ and hence the counit
of the adjunction $\Sigma \dashv \Omega$ gives us our map:
\[\epsilon : \Sigma (\Omega(K(\bZTwo,1))) \to_\star K(\bZ/2\bZ,1) \]

We would like to define $c_{0_k} := \epsilon$, but it is not entirely
obvious why this definition would define $c_x$ for \emph{all}
$x : \KTwoOne$ -- the type
$\Sigma (0_k = 0_k) \to_\star K(\bZ/2\bZ,1)$ is not a proposition but
a set, and hence this is not automatic. The trick is to add some
structure to the type of $c_x$ by instead considering the following type:
\begin{align}
  \sum_{e : \Sigma (0_k = x) \to_\star K(\bZ/2\bZ,1)} (e \neq \mathsf{const}) \label{eq:bigtype}
\end{align}
\begin{lemma}\label{lem:contr-fun-type}
  The type in \eqref{eq:bigtype} is contractible. Furthermore,
  $\epsilon$ is non-constant and thus is the centre of contraction
  when $x$ is $0_k$.
\end{lemma}
\begin{proof}
  Since we are proving a proposition, it suffices to do so when $x$ is
  $0_k$. We get
  \begin{align*}
  \Sigma (0_k = 0_k) \to_\star \KTwoOne &\simeq \Omega (\KTwoOne) \to_\star \Omega (\KTwoOne)\\
  &\simeq \mathbb{S}^0 \to_\star \mathbb{S}^0 \\
  &\simeq \mathsf{Hom}(\bZ/2\bZ,\bZ/2\bZ)
  \end{align*}
  By construction, this equivalence sends $\epsilon$ to the identity
  on $\bZ/2\bZ$. The predicate $(-) \neq \mathsf{const}$ is easily
  seen to be preserved by this chain of equivalences, and hence we get
  \[\sum_{e : \Sigma (0_k = 0_k) \to_\star K(\bZ/2\bZ,1)} (e \neq \mathsf{const}) \simeq \sum_{\phi : \mathsf{Hom}(\bZ/2\bZ,\bZ/2\bZ)} (\phi \neq \mathsf{const}) \]
  Since the identity is the unique non-constant map in
  $\mathsf{Hom}(\bZ/2\bZ,\bZ/2\bZ)$, we are done.
\end{proof}
Hence, by Lemma~\ref{lem:contr-fun-type}, we construct our family
$c_x : \Sigma(0_k = x) \to_\star \KTwoOne$ by choosing the unique
element of \eqref{eq:bigtype}.  This gives us our class
$e :H^1(\KTwoOne,\bZ/2\bZ)$. In fact, with this rather explicit
construction it is easy to show that $e = \trunc{\mathsf{id}}$, but
this additional knowledge will not be needed here. We may now
instantiate the Gysin sequence. We get, for $i \geq 1$, exact
sequences
\[\begin{tikzcd}[ampersand replacement=\&]
	{H^{i-1}(E,\bZ/2\bZ)} \& {H^{i-1}(\RPinf,\bZ/2\bZ)} \& {H^i(\RPinf,\bZ/2\bZ)} \& {H^i(E,\bZ/2\bZ)}
	\arrow["{(-)\smile e}", from=1-2, to=1-3]
        \arrow[from=1-1,to=1-2]
	\arrow[from=1-3, to=1-4]
\end{tikzcd}\]
where, recall, $\RPinf := \KTwoOne$ and $E := \sum_{x: \KTwoOne}(0_k = x)$. Since $E$ is contractible we get that the $(-)\smile e : {H^{i-1}(\RPinf,\bZ/2\bZ)} \to {H^i(\RPinf,\bZ/2\bZ)} $ is an isomorphism. Since $\RPinf$ is connected, we have $H^0(\RPinf,\bZ/2\bZ) \cong \bZ/2\bZ$, and hence we get a chain of isomorphisms
\[\bZ/2\bZ \cong H^0(\RPinf,\bZ/2\bZ) \cong H^1(\RPinf,\bZ/2\bZ) \cong \dots \cong H^n(\RPinf,\bZ/2\bZ)\]
whose composition is simply the map $(-)\smile e^n : \bZ/2\bZ \to H^n(\RPinf,\bZ/2\bZ)$. Hence, we have computed $H^*(\RPinf,\bZ/2\bZ)$.
\begin{theorem}
  $H^*(\RPinf,\bZ/2\bZ) \cong \bZ/2\bZ[x]$
\end{theorem}

%\anders{Jag kan inte hjälpa att tycka det är lite lustigt att det här är
%  så komplicerat... Ett direkt bevis är alltså inte möjligt? -- Kanske med den typiska modellen av $RPinf$ som CW-complex i oändlig dimension. Men det är inte sj}


==> sections/longabstract.tex <==
In his 2016 proof of $\pi_4(S^3) \cong \bZ/2\bZ$,
Brunerie~\cite{Brunerie16} crucially uses---but never proves---that
the smash product is symmetric monoidal. Due to the vast amount of
path algebra involved when reasoning about smash products, this has
since remained open. While it turns out that smash products are not
needed for Brunerie's proof~\cite{BrunerieNumber,BLM22}, the problem
is still interesting in its own right.  Several attempts have been
made at salvaging the situation. Floris Van Doorn~\cite{FlorisPhd}
came very close to a complete proof by considering an argument using
closed monoidal categories but left a gap where the path algebra got
too technical. Another line of attack by
Cavallo~and~Harper~\cite{CavalloHarper20, Cavallo21} is the addition
of parametricity. This provides a solution at the
cost of complicating the type theory. In this talk, we introduce a
heuristic for reasoning about functions defined over smash products
and use it to give a complete proof of the fact that the smash product
is symmetric monoidal. While all key results have been formalised
in \CubicalAgda\footnote{The formalisation is available at \url{https://github.com/aljungstrom/cubical/blob/pentagon/Cubical/HITs/SmashProduct/SymmetricMonoidal.agda} (L562). Note that the definition of \emph{precategories} is non-standard.}, the argument is in plain Book HoTT.

The model of the smash product we will use here is given by the cofibre of the inclusion $A \vee B \hookrightarrow A \times B$. For the sake of clarity, let us spell this out in detail: 
\begin{definition}
  The smash product of two pointed types $A$ and $B$ is the HIT generated by
  \begin{center}
  \begin{minipage}{5cm}
  \begin{itemize}
  \item a point $\star_\wedge : A \wedge B$
  \item for every pair $(a,b) : A \times B$, a point $\smashinc{a}{b} : A \wedge B$
  \end{itemize}
  \end{minipage}
  \begin{minipage}{9cm}
  \begin{itemize}
  \item for every point $a : A$, a path $\pushl{a}:\smashinc{a}{\star_B} = \star_\wedge$
  \item for every point $b : B$, a path $\pushr{b} : \smashinc{\star_a}{b} = \star_\wedge$
  \item a coherence $\pushlr : \pushl{\star_A} = \pushr{\star_B}$.
  \end{itemize}
  \end{minipage}
  \end{center}
\end{definition}
The fact that the smash product is commutative is very direct. Its
associativity, however, is harder to prove. This was first proved, in HoTT, by van
Doorn~\cite{FlorisPhd}, using the adjunction $(A \wedge B \to_\star C) \simeq (A \to_\star (B \to _\star C))$ and by Brunerie~\cite{brunerie18}, using a computer generated proof in
\Agda. Here, we give an explicit proof by considering a more involved HIT $\bigwedge(A,B,C)$ satisfying $(A \wedge B) \wedge C \simeq \bigwedge(A,B,C)$ and (trivially) $\bigwedge(A,B,C) \simeq \bigwedge(C,A,B)$. This automatically gives the desired equivalence $\alpha_{A,B,C} :  (A \wedge B) \wedge C \simeq A \wedge (B \wedge C)$. The advantage of this explicit description of the equivalence is that it becomes easier to trace. In particular, it is easy to understand its behaviour when applied to homogeneous points and $1$-dimensional path constructors. This will turn out to be precisely what we need.

The key problem in proving the fact that the smash product is symmetric monoidal is verifying MacLane's pengaton, i.e. the (pointed) commutativity of the following diagram.
\[\begin{tikzcd}[ampersand replacement=\& , row sep=.23cm]
	\& {((A \wedge B) \wedge C) \wedge D} \\
	{(A \wedge (B \wedge C)) \wedge D} \&\& {(A \wedge B) \wedge (C \wedge D)} \\
	{A \wedge ((B \wedge C) \wedge D)} \&\& {A \wedge (B \wedge (C \wedge D))}
	\arrow["{\alpha_{A,B,C} \wedge 1_D}"', from=1-2, to=2-1]
	\arrow["{\alpha_{A,B\wedge C,D}}"', from=2-1, to=3-1]
	\arrow["{\alpha_{A\wedge B,C,D}}", from=1-2, to=2-3]
	\arrow["{\alpha_{A,B,C\wedge D}}", from=2-3, to=3-3]
	\arrow["{1_A\wedge\alpha_{B, C,D}}", from=3-1, to=3-3]
	%% {A \wedge (B \wedge (C \wedge D))} \&\& {A \wedge ((B \wedge C) \wedge D)} \\
	%% \\
	%% {(A \wedge B) \wedge (C \wedge D)} \&\& {(A \wedge (B \wedge C)) \wedge D} \\
	%% \& {((A \wedge B) \wedge C)\wedge D}
	%% \arrow["{\alpha_{A,B\wedge C,D}}", from=1-3, to=3-3]
	%% \arrow["{\alpha_{A,B,C} \wedge \mathsf{id}_D}", from=3-3, to=4-2]
	%% \arrow["{\alpha_{A \wedge B,C,D}}"', from=3-1, to=4-2]
	%% \arrow["{\alpha_{A,B,C\wedge D}}"', from=1-1, to=3-1]
	%% \arrow["{\mathsf{id}_A \wedge \alpha_{B,C,D}}", from=1-1, to=1-3]
\end{tikzcd}\]
A naive proof attempt by smash product induction forces us to fill
(highly non-trivial) cubes up to $5$ dimensions and quickly descends
into coherence hell. It turns out that we never need to verify any
coherences coming from the $\pushlr$ constructor, but this still is
not enough. We need a stronger induction principle.
%% \begin{lemma}\label{lem:fst-coh}
%%   Let $A\,\tilde{\wedge}\,B$ denote the cofibre of the inclusion $A + B
%%   \to A \times B$ (this is precisely $A \wedge B$ without the
%%   $\pushlr$ constructor). The inclusion
%%   $\iota : A\,\tilde{\wedge}\,B \to A \wedge B$ equalises $f$ and $g$.
%% \end{lemma}
%% Informally, \cref{lem:fst-coh} tells us that we never have
%% to worry about the $\pushlr$ constructor when proving identities of
%% functions defined over smash products.
%
To this end, we recall that a pointed type $A$ is
called \emph{homogeneous} if for any point $a:A$ we have an equality
of pointed types $(A,\star_A) = (A,a)$. We turn our attention to an
incredibly useful lemma, first conjectured for Eilenberg-MacLane
spaces in work leading up to~\cite{BLM22} and later proved and
generalised by Cavallo (and later further generalised by~Buchholtz,
Christensen, G. Taxerås Flaten and Rijke~\cite{taxeras}) which states that any two pointed functions $f,g : A \to_\star B$ with $B$ homogeneous are equal as pointed functions iff their underlying functions are equal. 
Using the fact that $A \to_\star B$ is homogeneous whenever $B$ is, the adjunction $(A \wedge B \to_\star C) \simeq (A \to_\star (B \to _\star C))$ yields the following result.
\begin{lemma}\label{lem:evan-smash}
  Let $f,g : A \wedge B \to_\star C$ with $C$ homogeneous. We have $f = g$ as pointed functions iff $f\smashinc{a}{b} = g\smashinc{a}{b}$ for $(a,b) : A \times B$.
\end{lemma}
If we could apply \cref{lem:evan-smash} to functions $((A \wedge B) \wedge C) \wedge D \to A \wedge (B
\wedge (C \wedge D)) $, the
pentagon would be trivial. Unfortunately, arbitrary smash
products are \emph{not} necessarily homogeneous. Fortunately, there is still some use for the lemma. Let us consider the following construction.
\begin{definition}
  Let $f,g : A \wedge B \to C$ and $h : ((a , b) : A \times B) \to f\smashinc{a}{b} = g\smashinc{a}{b}$. We define two pointed functions $L_h : A \to_\star f(\star_\wedge) = g(\star_\wedge)$ and $R_h : B \to_\star f(\star_\wedge) = g(\star_\wedge)$ by
  \begin{align*}
    L_h(a) &= (\ap{f}{\pushl{a}})^{-1} \cdot h(a,\star_B) \cdot \ap{g}{\pushl{b}} \\
    R_h(b) &= (\ap{f}{\pushr{b}})^{-1} \cdot h(\star_A,b) \cdot \ap{g}{\pushr{b}} 
  \end{align*}
  where we may simply take $f(\star_\wedge) = g(\star_\wedge)$ to be pointed by either $L_h(\star_A)$ or $R_h(\star_A)$ (these are equal by $\pushlr$, so the choice does not matter).
\end{definition}
We can easily derive the following induction principle.
\begin{lemma}\label{lem:main}
  Let $f ,g: A \wedge B \to C$. The following data gives an equality $f = g$:
  \begin{itemize}
  \item A homotopy $h : ((a , b) : A \times B) \to f\smashinc{a}{b} = g\smashinc{a}{b}$
  \item Equalities of pointed functions $L_h = \mathsf{const}_{L_h(\star_B)}$ and $R_h = \mathsf{const}_{R_r(\star_B)}$.
  %% \item (Optional, if an equality of pointed functions is desired): A coherence $\star_f = F_h(\star_B) \cdot \star_g$
  \end{itemize}
\end{lemma}
The second datum above looks almost absurd: it is asking us to provide
equalities of pointed functions, which is much stronger than what is
actually needed. However, the codomain of these functions is
homogeneous, so we need not worry. In particular, when
e.g. $A$ is another smash product, as is the case in the pentagon,
\cref{lem:evan-smash} applies which in effect makes this part of the proof trivial. In fact, \cref{lem:main} and \cref{lem:evan-smash} may be iteratively applied to any $n$-fold smash product, completely removing the need to verify any higher coherences. Let us state this as an informal theorem:
\begin{theorem}[Informal]\label{thm:informal}
  To show that two functions $f,g : ((A_1 \wedge A_2) \wedge \dots) \wedge A_n \to B$ are equal, it suffices to provide a family of paths $f \langle x_1,\dots,x_n \rangle = g \langle x_1 , \dots,x_n\rangle$ for $x_i : A_i$ and to show that this is coherent with $f$ and $g$ on any \textbf{single} application of $\pushll$ or $\pushrr$.
\end{theorem}
This applies to all non-trivial proofs related to the symmetric monoidal structure of the smash product, and in particular to the pentagon. The pentagon holds by definition for homogeneous elements $\langle a,b,c,d \rangle : ((A \wedge B) \wedge C) \wedge D$, so we are only left to trace single instances of the $\mathsf{push}$ constructors, which turns out to be very direct (albeit somewhat lengthy). The pointedness requirement is equally direct. \cref{thm:informal} can be used to show the remaining axioms and we easily arrive at the main result: 
  \begin{theorem}
    The smash product is symmetric monoidal with the type of booleans
    as unit.
  \end{theorem}


